PIMMiner: A High-performance PIM Architecture-aware Graph Mining Framework

Graph mining applications, such as subgraph pattern matching and mining, are widely used in real-world domains such as bioinformatics, social network analysis, and computer vision. Such applications are considered a new class of data-intensive applications that generate massive irregular computation workloads and memory accesses, which degrade the performance significantly. Leveraging emerging hardware, such as process-in-memory (PIM) technology, could potentially accelerate such applications. In this paper, we propose PIMMiner, a high-performance PIM architecture graph mining framework. We first identify that current PIM architecture cannot be fully utilized by graph mining applications. Next, we propose a set of optimizations and interfaces that enhance the locality, and internal bandwidth utilization and reduce remote bank accesses and load imbalance through cohesive algorithm and architecture co-designs. We compare PIMMiner with several state-of-the-art graph mining frameworks and show that PIMMiner is able to outperform all of them significantly.

==> section/3_Motivation_old.tex <==
\label{sec:motivation}

\iffalse

\subsection{Limitations of CPU Acceleration}
\label{subsec:moti-cpu}
% \subsection{Scalability issue of GPMI application}
In this section, we identify the limitations of GPMI on CPUs in terms of multi-threading and LLC cache effectiveness.
We run seven graphs (described in Table~\ref{tab:Graph Datasets}) on a 96 hyperthreaded CPU (48 physical cores).
The details of our graphs and CPU are in section~\ref{subsec:setup}.
%To reduce the load imbalance problem, we only schedule and execute one vertex $v_0$ at a time.
We take 4-clique counting (4-CC) as an example, and other application trends are similar to 4-CC.

\noindent \textbf{Limitations of multithreading.}
Figure~\ref{fig:4-CC speedup cpu} shows the speedup of the \emph{nest\_for\_loop} function (in Figure \ref{fig:AutoMine}) from a single thread to 128 threads.
Since graph \emph{CiteSeer} and \emph{P2P} are too small, the execution time is unstable when multi-threaded, so we do not count the speedup of these two graphs in Figure~\ref{fig:4-CC speedup cpu}.
Because the size of \emph{LiveJournal} is large, the speedup from multi-threading is high.
In Figure~\ref{fig:4-CC speedup cpu}, the speedup of 4-CC scales well from 1 thread to 32 threads and becomes stable with more than 32 threads.
This is because of the limited CPU computing resources (e.g., physical core number is 48 in the machine) -- when the number of threads reaches a certain number, increasing the number of threads has little effect on program performance improvement.


 
\begin{figure}[t]
\centering 
\vspace{-0.1cm}
\includegraphics[width=0.75\linewidth]{pic/4-CC_speedup2.pdf}
\vspace{-0.4cm}
\caption{4-CC Pattern Speedup on CPU.} 
\label{fig:4-CC speedup cpu}
%\vspace{-0.3cm}
\end{figure}


% \textbf{Ineffective LLC cache.}
\noindent \textbf{Poor LLC locality.}
Table~\ref{tab:4-cc LLC miss} shows the LLC cache miss rate when 4-CC runs on the CPU. 
The data is collected with \textit{perf tool} when running with 96 threads.
%We choose 96 threads because our CPU has 96 hyperthreads, and the program performs well with 96 threads in Figure~\ref{fig:4-CC speedup cpu}.
In Table~\ref{tab:4-cc LLC miss}, for the 4 large graphs \emph{Mico}, \emph{Youtube}, \emph{Patents} and \emph{LivaJournal}, the LLC cache miss rate is between 20\% and 50\%, which is relatively large.
Therefore, the memory access intensity from GPMI is high. 
In addition, the access pattern is irregular due to frequent vertex traversal.



\begin{table}[t]
	\centering  % 显示位置为中间
	\small
	\vspace{-0.1in}
	\caption{4-CC LLC miss rate on CPU with 96 threads.}  % 
	\label{tab:4-cc LLC miss}  % 用于索引表格的标签
	\vspace{-0.1in}
	\resizebox{0.8\linewidth}{!}{
	\begin{tabular}{c|c|c|c|c|c|c|c}  
	\hline
	    Graph & CI & PP & AS & MI & YT & PA & LJ \\
		\hline  % 表格的横线
		LLC miss rate (\%) & 13.4 & 9.0 & 5.2 & 30.8 & 24.1 & 54.7 & 38.1 \\
		\hline
	\end{tabular}
	}
\end{table}


Due to the poor scalability of the CPU, to further improve the performance of GPMI, we need a new architecture with more cores and better scalability. In addition, because of the poor locality of GPMI memory accesses, the new architecture does not require multiple cache levels. Based on these two properties, we find that PIM architecture is well-suited for GPMI.
The number of cores and memory size in one HBM-PIM stack is 128 and 4GB, respectively. If needed, the system can use up to 4 stacks for higher scalability. Compared to CPU, there are more physical cores in PIM architecture, although the PIM cores are not as powerful as CPU cores. 
Besides, PIM is best for memory-intensive applications with poor locality, with only L1 cache, it can reduce the miss penalty for an L1 miss without going through multiple-level caches.



\fi


% 1. CPU performance doesn't scale well with increasing threads
% (4-CC)

% 2. LLC miss rate is high(96 threads)
% (4-CC)


% \begin{table}[!h]
% 	\centering  % 显示位置为中间
% 	\small
% 	\vspace{-0.1in}
% 	\caption{MPKI in different graphs and applications}  % 表格标题
% % 	\caption{Graph Datasets~\cite{mawhirter2019automine} 5\% Deg. = the top 5\% node degrees / all node degrees.}  % 表格标题
% 	\label{tab:MPKI}  % 用于索引表格的标签
% 	%字母的个数对应列数，|代表分割线
% 	% l代表左对齐，c代表居中，r代表右对齐
% 	\vspace{-0.1in}
% 	\resizebox{\linewidth}{!}{
% 	\begin{tabular}{c|c|c|c|c}  
% 	\hline
% 	    \textbf{Graph} & 3-CC & 4-CC & 5-CC & 3-MC\\
% 		\hline  % 表格的横线
% 	    CiteSeer(CI) & 1.55 & 1.74 & 1.94 & 1.16  \\ 
% 	    P2P(PP) & 0.57 & 0.62 & 0.62 & 0.39\\
% 	    Astro(AS) & 0.22 & 0.03 & 0.01 & 0.15 \\
% 		MiCo(MI) & 1.28 & 0.05 & 0.03 & 0.86  \\
% 		com-Youtube(YT) & 9.50 & 4.99 & 0.56 & 5.08  \\
% 		cit-Patents(PA) & 8.40 & 6.01 & 0.17 & 6.24 \\
% 		soc-LiveJournal1(LJ) & 12.66 & 1.27 & 0.22 & 8.33  \\
% 		\hline
% 	\end{tabular}
% 	}
% \end{table}

NDMiner \cite{talati2022ndminer} discusses the characteristics of GPMI in detail, and gives the conclusion that PIM is suitable for calculating GPMI.
But NDMiner puts the processing unit outside the dram bank, which is different from the HBM-PIM proposed by Samsung recently. In this section we will run GPMI on Samsung's HBM-PIM and analyze its results.

\subsection{Baseline PIM Performance}


\begin{table}[t]
	\centering  % 显示位置为中间
	\small
	% \vspace{-0.1in}
	\caption{Performance between 96-threads CPU (L3 cache) and 128-core PIM (L1 cache) in 4-CC.}  % 表格标题
	\label{tab:Performance 128-core CPU and 128-core PIM 4-CC}  % 用于索引表格的标签
	%字母的个数对应列数，|代表分割线
	% l代表左对齐，c代表居中，r代表右对齐
	% \vspace{-0.1in}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{c|c|c|c|c|c|c}  
	\hline
	    Graph & Processing & Execution & Average  & Exe/Avg & Execution & Average \\
	     & Unite & Time (s) & Time (s) & & Speedup & Speedup \\
		\hline  % 表格的横线
	    \multirow{2}{*}{CI} & CPU & 3.80E-05 & 1.65E-05 & 2.30   & \textbf{\multirow{2}{*}{0.92x}} &\textbf{\multirow{2}{*}{0.46x}} \\
	    & PIM & 4.13E-05 & 3.57E-05 & 1.16   & & \\
	    \hline
		\multirow{2}{*}{PP} & CPU & 7.07E-04 & 3.37E-04 & 2.10   & \multirow{2}{*}{4.15x} &\multirow{2}{*}{2.16x} \\
		& PIM & 1.71E-04 & 1.56E-04 & 1.09  &  & \\
		\hline
		\multirow{2}{*}{AS} & CPU & 1.04E-02 & 7.04E-03 & 1.48   & \multirow{2}{*}{2.58x} &\multirow{2}{*}{2.92x} \\
		& PIM & 4.05E-03 & 2.41E-03 & 1.68 & & \\
		\hline
		\multirow{2}{*}{MI} & CPU & 1.64E-01 & 8.48E-02 & 1.93   & \textbf{\multirow{2}{*}{0.39x}} & \textbf{\multirow{2}{*}{0.51x}} \\
		& PIM & 4.22E-01 & 1.66E-01 & 2.53  &  & \\
		\hline
		\multirow{2}{*}{YT} & CPU & 1.49E-01  & 9.18E-02  & 1.63 & \textbf{\multirow{2}{*}{0.08x}} & \textbf{\multirow{2}{*}{0.24x}} \\
		& PIM & 1.83 & 3.78E-01 &  4.84  &  & \\
		\hline
		\multirow{2}{*}{PA} & CPU & 1.83E-01 & 1.37E-01 & 1.34  & \multirow{2}{*}{2.66x} & \multirow{2}{*}{2.53x} \\
		& PIM & 6.89E-02 & 5.40E-02 & 1.28   &  & \\
		\hline
		\multirow{2}{*}{LJ} & CPU & 3.09  & 2.59  & 1.19  & \textbf{\multirow{2}{*}{0.03x}} & \textbf{\multirow{2}{*}{0.56x}} \\
		& PIM & 103.13 & 4.63  & 22.29 &  & \\
		\hline
	\end{tabular}
	}
	\vspace{-0.2in}
\end{table}

% Based on the observations in Section \ref{subsec:moti-cpu}, we believe that GPMI applications could potentially gain benefits from PIM architecture.
% Therefore, 
We run 4-CC on PIM and compare the results of CPU in Table~\ref{tab:Performance 128-core CPU and 128-core PIM 4-CC}.
We sort the vertices in the descending order of degree.
To ensure the balance of the size of the neighbor list $N(v)$ in each PIM unit, we use the round-robin method to store the neighbor lists, which is commonly used in related work \cite{talati2022ndminer,su2021exploring}.
%According to the vertex id $v$, we store the neighbor lists $N(v)$ in different PIM units sequentially.Assuming there are $N_{pim}$ PIM units, PIM Unit $n$ will store the neighbor lists $N(v)$ of $v=n,n+N_{pim},n+2*N_{pim},...$.
The CPU performance is measured on a real system, and the PIM performance is measured from a cycle-accurate simulator. The details of our experimental methodologies are in Section~\ref{subsec:setup}.
To reduce the overhead of OpenMP, CPU execution time and CPU average time are measured inside OpenMP \emph{for} loop.
We report execution time as the program finish time among the whole cores, as well as the average time that each core spent to run the program.

Based on the results from Table \ref{tab:Performance 128-core CPU and 128-core PIM 4-CC}, we find that the performance gain of PIM is \textit{not} consistent -- could be better or worse than the CPU, regardless of the graph size.
Additionally, we compute the ratio of execution time to average time (Exe/Avg) on CPU and PIM to measure the load imbalance.
Both CPU and PIM have load imbalance issues, and PIM has more severe issue, especially for graph \emph{LiveJournal}, whose execution time is 22 times over average time.


The load imbalance mainly comes from the loop iteration to core mapping. From Figure~\ref{fig:AutoMine}, we know that finding
$n$-size patterns requires $n$ layers of \textit{for} loops. When executing the code on multiple cores, the most straightforward way is to assign the intersection and subtraction (I/S) operations (the second \textit{for} loop to the last \textit{for} loop) to the same core base on the root vertex ($v_0$ in the first-level loop). Such a method (root vertex-based assignment) can guarantee the data dependency of following I/S operations. 
However, the number of loops at each layer is determined by the \textit{{results}} of I/S operations (e.g., $N(v_0)-N(v_1)$ in Figure~\ref{fig:AutoMine}), which varies a lot based on patterns or graphs, and cannot be determined by offline profiling.
In comparison, for general graph processing applications such as BFS and PR, the workload of each vertex is small and easy to obtain from the vertex degree.
Therefore, compared with general graph processing applications, the workloads of GPMI applications on different cores could differ significantly.
As the matching size increases, the number of layers of the \textit{for} loop increases, resulting in a more significant load imbalance. 




%\cb{The reason for load imbalance is discussed in \cite{su2021exploring}.}
\noindent \textbf{Key takeaway.} Although PIM could theoretically improve GPMI applications with low latency and high bandwidth memory accesses, directly offloading the GPMI execution kernel to PIM cannot guarantee performance speedup. The graph mining framework should be PIM architecture-aware to leverage the fast near-core memory accesses. 


% % Since our machine has 96 processors, so we choose 96 threads.
% To reduce the overhead of OpenMP, our execution time and average time are recorded in the for loop.


% Time in OpenMP
% \begin{table}[!h]
% 	\centering  % 显示位置为中间
% 	\small
% 	\vspace{-0.1in}
% 	\caption{Performance between 96-threads CPU (L3 cache) and 128-core PIM (L1 cache) in 3-CC.}  % 表格标题
% 	\label{tab:Performance 128-core CPU and 128-core PIM 3-CC}  % 用于索引表格的标签
% 	%字母的个数对应列数，|代表分割线
% 	% l代表左对齐，c代表居中，r代表右对齐
% 	\vspace{-0.1in}
% 	\resizebox{\linewidth}{!}{
% 	\begin{tabular}{c|c|c|c|c|c}  
% 	\hline
% 	    Graph & Processing Unite & Execution Time (s) & Avg Time (s) & Exe/Avg & Speedup\\
% 		\hline  % 表格的横线
% 	    \multirow{2}{*}{CI} & CPU & 1.22E-04 & 7.85E-05 & 1.55 & \multirow{2}{*}{3.66x} \\
% 	    & PIM & 3.33E-05 & 2.84E-05 & 1.17 & \\
% 	    \hline
% 		\multirow{2}{*}{PP} & CPU & 1.24E-03 & 1.03E-03 & 1.20 & \multirow{2}{*}{7.60x} \\
% 		& PIM & 1.63E-04 & 1.50E-04 & 1.08 &\\
% 		\hline
% 		\multirow{2}{*}{AS} & CPU & 3.21E-03 & 2.23E-03 & 1.44 & \multirow{2}{*}{2.94x} \\
% 		& PIM & 1.09E-03 & 9.70E-04 & 1.13 &\\
% 		\hline
% 		\multirow{2}{*}{MI} & CPU & 1.51E-02 & 1.05E-02 & 1.43 & \multirow{2}{*}{1.98x} \\
% 		& PIM & 7.62E-03 & 6.11E-03 & 1.25 &\\
% 		\hline
% 		\multirow{2}{*}{YT} & CPU & 1.51E-02 & 1.05E-02 & 1.51 & \multirow{2}{*}{0.43x} \\
% 		& PIM & 1.70E-01 & 1.22E-01 & 1.39 &\\
% 		\hline
% 		\multirow{2}{*}{PA} & CPU & 2.26E-01 & 1.74E-01 & 1.30 & \multirow{2}{*}{3.29x} \\
% 		& PIM & 6.87E-02 & 5.96E-02 & 1.15 &\\
% 		\hline
% 		\multirow{2}{*}{LJ} & CPU & 7.67E-01 & 5.49E-01 & 1.40 & \multirow{2}{*}{0.70x} \\
% 		& PIM & 1.10  & 5.98E-01 & 1.83 &\\
% 		\hline
% 	\end{tabular}
% 	}
% \end{table}

% \begin{table}[!h]
% 	\centering  % 显示位置为中间
% 	\small
% 	\vspace{-0.1in}
% 	\caption{Performance between 96-threads CPU (L3 cache) and 128-core PIM (L1 cache) in 3-MC.}  % 表格标题
% 	\label{tab:Performance 128-core CPU and 128-core PIM 3-MC}  % 用于索引表格的标签
% 	%字母的个数对应列数，|代表分割线
% 	% l代表左对齐，c代表居中，r代表右对齐
% 	\vspace{-0.1in}
% 	\resizebox{\linewidth}{!}{
% 	\begin{tabular}{c|c|c|c|c|c}  
% 	\hline
% 	    Graph & Processing Unite & Execution Time (s) & Avg Time (s) & Exe/Avg & Speedup\\
% 		\hline  % 表格的横线
% 	    \multirow{2}{*}{CI} & CPU & 1.81E-04 & 9.69E-05 & 1.87  & \multirow{2}{*}{1.70x} \\
% 	    & PIM & 1.06E-04 & 6.88E-05 & 1.55  & \\
% 	    \hline
% 		\multirow{2}{*}{PP} & CPU & 1.16E-02 & 1.95E-03 & 5.96  & \multirow{2}{*}{25.08x} \\
% 		& PIM & 4.63E-04 & 4.16E-04 & 1.11  &\\
% 		\hline
% 		\multirow{2}{*}{AS} & CPU & 5.75E-03 & 4.04E-03 & 1.42  & \multirow{2}{*}{1.74x} \\
% 		& PIM & 3.30E-03 & 2.78E-03 & 1.19  &\\
% 		\hline
% 		\multirow{2}{*}{MI} & CPU & 5.45E-02 & 2.63E-02 & 2.08  & \multirow{2}{*}{1.96x} \\
% 		& PIM & 2.79E-02 & 1.71E-02 &  1.63 &\\
% 		\hline
% 		\multirow{2}{*}{YT} & CPU & 1.16  & 1.55E-01 & 7.48  & \multirow{2}{*}{0.19x} \\
% 		& PIM & 6.07 & 2.78E-01 & 21.83  &\\
% 		\hline
% 		\multirow{2}{*}{PA} & CPU & 5.45E-01 & 4.01E-01 & 1.36  & \multirow{2}{*}{1.78x} \\
% 		& PIM & 3.07E-01 & 2.05E-01 & 1.50  &\\
% 		\hline
% 		\multirow{2}{*}{LJ} & CPU & 2.34  & 1.60  & 1.46  & \multirow{2}{*}{0.47x} \\
% 		& PIM & 4.99  & 1.34  & 3.73  &\\
% 		\hline
% 	\end{tabular}
% 	}
% \end{table}




==> section/4_Framework.tex <==
\label{sec:PIMMiner Design}


\subsection{Overview}
\vspace{-0.05in}
In this section, we present the PIMMiner, an enhanced graph mining framework that can fully utilize general PIM architecture for performance acceleration. PIMMiner includes four main optimizations: conditional access filter, local-first data mapping, critical data duplication, and PIM-aware workload stealing. We show the high-level overview of this framework in Figure \ref{fig:PIMMiner}. 
We incorporate a simple hardware component called conditional filter(details in \S \ref{subsec:filter}) with each PIM unit.
Then, data management schemes for better locality are applied to the data in the memory bank.
We also store metadata tables used for workload stealing in the memory bank in a distributed way.
We next describe the design details of our proposed schemes.

\begin{figure}[t]
\centering 
\includegraphics[width=1\linewidth]{pic/PIMMinerv7.pdf}
\vspace{-0.5cm}
\caption{PIMMiner framework overview.} 
\label{fig:PIMMiner}
\vspace{-0.5cm}
\end{figure}

%  \hl{Maybe just keep one channel on the left. Right part is hard to read from the figure}
 

% According to the characteristics of GPMI algorithm and PIM architecture, we propose 4 improvement measures:
% Memory Access Filtering, PIM Address Mapping, Data Copying, Work Stealing.
% These improvements are not only applicable to GPMI, but also to other algorithms.
% For example, memory access filtering can be used in graph sampling, and new addressing mapping and data copying are applicable to all PIM programs.

\vspace{-0.05in}
\subsection{Conditional Access Filter}\label{subsec:filter}

\vspace{-0.05in}


According to the GPMI algorithm, when accessing the neighbor lists ($N(v)$), the program only needs a part of neighbor vertices for computation due to symmetry breaking.
For example, in Figure~\ref{fig:AutoMine}, the program only needs vertices in $N(v_0)-N(v_1)$ that have smaller id than $v_1$.
In conventional memory architectures, there are no processing units in memory, so unnecessary memory accesses are sent to the host CPU and cannot be removed in advance.
With PIM, before sending the data for computation, the PIM unit can read the data in advance and filter out the data that do not meet the conditions, thereby reducing data transmission.


\begin{figure}[t]
\centering 
\includegraphics[width=0.4\textwidth]{pic/PIMMiner_Filter.pdf}
\vspace{-0.3cm}
\caption{Conditional access filter.} 
\label{fig:Filter}
\vspace{-0.5cm}
\end{figure}


In our PIMMiner framework, to reduce the interference of memory access filter on PIM units, we add lightweight hardware dedicated to filter unnecessary data on PIM units, as shown in Figure~\ref{fig:PIMMiner} (gray part).
Our conditional filter is designed to handle the memory accesses with bounded data.
The detail of our conditional access filter is shown in Figure~\ref{fig:Filter}.
One 32-bit filter contains one subtractor, one filter logic, and two registers.
When the bank receives a memory access request to the neighbor list $N(v)$, if there are restrictions in memory request, the bank will extract the threshold $th$ and the comparison parameter $cmp$ from the memory request and store them in the two registers (dark blue squares in Figure~\ref{fig:Filter}) respectively.
Then, the filter reads the data $v_x$ from sense amplifier.
$v_x$ is first sent to the subtractor and subtracted with $th$ ($v_x-th$).
The result (1 is positive, 0 is equal, -1 is negative) will be sent to filter logic.
In filter logic, if the result matches the condition $cmp$, output data $v_x$; otherwise, filter out the data.
In this way, only two clock cycles of latency are required for each data filter (one cycle for subtraction, one cycle for comparison).
In our experiment, the width of TSVs on PIM is 64 bits.
Since one filter can handle a 32-bit integer, to maximize TSV bandwidth utilization, we add two filters per bank, which can send 64-bit data per clock cycle.
%Therefore, we place two filters per PIM unit.


% \cb{
We assume that the data transferred between PIM units is organized as a packet, which is described in HMC specifications\cite{hmc2013hybrid}. 
A packet without data has 128 bits metadata, which is much smaller than the packet with data (128 bits + 64 Byte Data). In this design, if the data is filtered out, a packet without data is sent to the destination PIM unit; otherwise a packet containing the data pointed to by the address is sent.
% }
% \cb{
We add one bit in the memory request packet to distinguish whether the data is obtained directly or obtained through a filter, thereby helping the memory controller to obtain the data. If the filter is used, the memory request packet will also contain a threshold value and the comparison symbol (we use the less than sign here), and the filter will read vertex IDs according to the address for comparison. If the data is filtered out, we will respond with a packet with no data, otherwise respond with a packet containing the data in this address.
% }


Note that the conditional access filter design can be applied to other workloads that has comparisons, such as database selection operator\cite{kepe2019database}.









% to reduce the performance impact of memory access filtering on programs executed on PIM unites, we add an additional hardware to PIM unite to filter memory accesses, thereby reducing interaction with PIM unites.
% Figure~\ref{fig:PIMMiner} shows the detail of our filter hardware.
% Since there are 64-bit TSVs in our framework, our filter on each PIM unite has two sets of hardware.
% As shown in Figure~\ref{fig:PIMMiner}, each set of hardware contains one subtraction ALU, one controller, and two registers.


% In Figure~\ref{fig:PIMMiner}, assuming that PIM Core 0 executes $N(0)-N(5)$ instruction, if there is no filter, the memory access of N(0) is as shown in Baseline PIM, with 2 in-bank accesses, 2 in-channel accesses and 2 cross-channel accesses.
% But if we add a filter to each core, the filter restriction is $N(0)<v_1=5$.
% Then N(0) on bank group 2 will be all filtered out, N(0) on bank group 1 will be filtered out 5, and only 3 will be sent to PIM core 0.
% In this way, $N(0)$ has only 2 in-bank accesses and 1 cross-channel access.



\vspace{-0.05in}
\subsection{Local-First Data Mapping}
\label{subsec:Local-First Data Mapping}
\vspace{-0.05in}

%Unlike the traditional CPU memory architecture, the processing unit of PIM is in memory, not out of memory, so the conventional address mapping method is not suitable for PIM. To take full advantage of PIM locality, that is, high bandwidth and low latency within the same bank group, we propose a new address mapping method \emph{local-fisrt data mapping}.

Conventional memory address mapping for HBM maximizes bandwidth utilization by interleaving data across memory banks and channels. However, it is sub-optimal for PIM. In PIMMiner, we propose a new address mapping method \emph{local-fisrt data mapping}, aiming to exploit low-latency and high-bandwidth local memory bank accesses for PIM units.


\begin{figure}[t]
\centering 
\includegraphics[width=\linewidth]{pic/AddressMappingv1v3.pdf}
\vspace{-0.3cm}
\caption{Conventional and local-fist address mapping.} 
\label{fig:AddressMapping}
\vspace{-0.5cm}
\end{figure}

\paragraph{Conventional address mapping}
Conventional address mapping interleaves consecutive memory addresses into different channels to maximize the memory bandwidth to the host. 
As shown in Figure~\ref{fig:AddressMapping}, consecutive memory addresses are allocated to different channels first, then to different banks in the same channel, and finally to different bank groups.
In Figure~\ref{fig:AddressMappingv2}, we assume that there are two memory channels, $N(0)$ and $N(5)$ are mapped to different memory channels with the conventional address mapping. 
If CPU wants to access $N(0)$, then channel 0 and 1 can send \{1,2\} and \{3,5\} at the same time.
However, suppose the computation is on PIM unit 0,  although it can quickly access the local data in bank group 0 of channel 0 (blue dotted arrow), accessing the rest of $N(0)$ and $N(5)$ data in channel 1 through TSVs (red dotted arrow) are slower. 


\paragraph{Local-first data mapping}
We modify the memory address mapping to allow PIM units to access neighbor lists, which are consecutive memory blocks, from their local memory banks. The new address mapping scheme is shown in Figure \ref{fig:AddressMapping}.
Each neighbor list is stored in different channels and bank groups in sequence.
Assuming that there are two channels, and each channel has two bank groups, then in Figure \ref{fig:AddressMappingv2}, $N(0)$ is stored in bank group 0 of channel 0; $N(1)$ is stored in bank group 0 of channel 1; $N(2)$ is stored in bank group 1 of channel 0; and so on.
Using the same example in Figure \ref{fig:AddressMappingv2}, if PIM unit 0 needs to access the two neighbor lists $N(0)$ and $N(5)$, only $N(5)$ will be fetched from remote memory banks. In this way, PIM units can better exploit their local memory banks and reduce remote memory access substantially. 



\begin{figure}[t]
\centering 
\includegraphics[width=\linewidth]{pic/AddressMappingv6.pdf}
\vspace{-0.3cm}
\caption{Conventional and local-fist address mapping.} 
\label{fig:AddressMappingv2}
\vspace{-0.2cm}
\end{figure}




\vspace{-0.05in}
\subsection{Critical Data Duplication}
\vspace{-0.05in}
To further improve the usage of near-core local banks, we propose \emph{critical data duplication} that stores critical data in the unused memory space in the memory banks. 
This optimization can be done during the pre-processing time. 
We use Algorithm \ref{alg:Critical Data} to determine the \emph{border vertex} $v_b$ of critical data that could be stored in each memory bank. We find that vertices with high degrees have a higher chance of being reused. Therefore, we choose to keep them as critical data that is duplicated across multiple banks.
%Through \emph{local-first data mapping}, each neighbor list $N(v)$ is continuously stored in the same bank. 
When accessing memory, the memory controller can determine whether to access the duplication in the near-core bank ($v < v_b$) or access data from other banks ($v \geq v_b$).

\begin{algorithm}[!h]
\caption{Calculate Critical Data}
\label{alg:Critical Data}
\small
\begin{algorithmic}[]
\State{\textbf{Input:} \emph{Graph G}, \emph{Memory Size M}, \emph{PIM Unit Number $N_{pim}$}}; 
\State{\textbf{Output}: \emph{border vertex $v_b$}}.
\end{algorithmic}
\hline 
\begin{algorithmic}[1]
\State{Sort the vertices in \emph{G} in descending order of degree}
\State{\emph{FreeMem} $\gets$ \emph{M} - \emph{G.size}}
\State{\emph{FreeMemBG} $\gets$ \emph{FreeMem} / $N_{pim}$}
\State{\emph{UsedMemBG} $\gets$ 0}
\For{\emph{i} = 0 \textbf{to} \emph{G.v} - 1}
\If{(\emph{UsedMemBG} + \emph{G.$v_i$.neighborSize}) $\leq$ \emph{FreeMemBG} }
\State{\emph{UsedMemBG} $\gets$ \emph{UsedMemBG} + \emph{G.$v_i$.neighborSize}}
\Else{}
\State{break}
\EndIf
\EndFor 
\State{$v_b$ $\gets$ \emph{i}}
\end{algorithmic}
\end{algorithm}
% \vspace{-0.1in}

\noindent \textit{Implementation.}
Critical data duplication can be implemented during the pre-processing time. The compiler is able to map the addresses of duplicated neighbor list in the near-bank first. In this way, the memory controller can directly fetch the duplicated data without additional operations. 



\vspace{-0.05in}
\subsection{Workload Scheduler with Stealing}
\vspace{-0.05in}
\label{subsec:stealing}
Lastly, we propose a PIM-aware workload scheduler with stealing capability to address the load imbalance problems identified during the program execution. 
Each PIM unit will store two tables: \emph{execution table} $T_{exe}$, which stores the index of each level in \emph{for loop} being executed by this PIM unit; and \emph{schedule table} $T_{sch}$, which stores the index of each level in \emph{for loop} to be executed next. 
$n.T_{exe}[i]$ represents the index at level $i$ in the \emph{execution table} of PIM unit $n$.
% $n.T_{exe}[i]$ stores the index at level $i$ in the \emph{execution table} of PIM unit $n$.
The correspondence between $v_0$, $v_1$ and $v_2$ in Figure \ref{fig:AutoMine} and the index in tables is
$v_0 = T_{exe}[0], v_1 = N(v_0)[T_{exe}[1]], v_2 = N(v_1)[T_{exe}[2]]$, and so on.
$N(v)[i]$ represents the $i$-th neighbor vertex in the neighbor list of vertex $v$.
We describe the workload stealing and scheduling algorithm in Algorithm~\ref{alg:Stealing}.

% \vspace{-0.05in}

\paragraph{Scheduler Main Execution Flow (lines 1-10)}
First, we initialize the \emph{schedule table} of each PIM unit (line 1).
During program execution, the PIM unit first updates \emph{execution table} according to the \emph{schedule table} (line 3).
If \emph{execution table} $T_{exe}$ is empty (line 4), it means that every level in the table is \emph{NULL}, then PIM unit $n$ will try to steal some pending tasks from the \emph{schedule table} from other PIM units (line 5).
If all \emph{schedule tables} are empty, which means no tasks need to be executed, then PIM unit $n$ cannot steal any tasks.
In this case, we consider that PIM unit $n$ has finished all task, and should end. (lines 6,7).
After updating \emph{execution table}, if \emph{execution table} is not empty,  the PIM unit $n$ does not need to steal tasks from other PIM units, instead, 
it will first update \emph{schedule table}, then execute \emph{execution table} (lines 9-10).

% \vspace{-0.05in}

\paragraph{Initialize Schedule Table (lines 11-12)}
To increase near-core bank memory access, we choose the vertex $v$ whose neighbor list $n(v)$ is stored in the near-core banks as $v_0$ in \emph{schedule table}.
% in the same bank group with PIM unit as $v_0$ in \emph{schedule table}.
According to the mapping method in Section \ref{subsec:Local-First Data Mapping}, the neighbor list $N(v)$ of $v=n,n+N_{pim},n+2*N_{pim},...$ is stored on PIM unit $n$ ($N_{pim}$ is the number of PIM units), so we use $v_0 = n$ to initialize \emph{schedule table} (line 12), and add $N_{pim}$ when updating $v_0$ (lines 25,34).

\vspace{-0.05in}

\paragraph{Update Execution Table (lines 13-17)}
Each level of \emph{schedule table} stores the index to be executed in the next run to this level.
Updating \emph{execution table} is to obtain the index to be executed by the next task from \emph{schedule table}.
Because the last level (level $S-1$) of \emph{schedule table} stores the index to be executed that is closest to the currently executed index, the PIM unit will first search from the last level to the first level (line 14).
When the first non-null item $T_{sch}$[\emph{i}] is encountered,  $T_{sch}$[\emph{i}] is copied to $T_{exe}$[\emph{i}], and break.


% \vspace{-0.05in}

\paragraph{Steal Schedule Table (lines 18-29)}
To reduce the number of stealing, the PIM unit selects another unit with the largest amount of tasks to steal. And usually, the tasks in the first level are the largest (because the tasks of the following levels are included).
Stealing event needs to scan the \emph{schedule table} of other PIM units starting from the first level.
When a stealing event is triggered, PIM unit $n$ first sends a read request of \emph{schedule table} to all PIM units (line 19).
Then the PIM unit scans all \emph{schedule table} from the first level (line 20) and prioritizes the task whose neighbor list is stored in nearby banks (line 21).
After finding the task in unit $m$ to be stolen (line 22), the PIM unit $n$ copies the task to its own \emph{schedule table} $n.T_{sch}$ (line 23), and sends the updated table $m.T_{sch}$ to PIM unit $m$ (lines 24-27). 
At the same time, to ensure the correctness of task index at the previous level, PIM unit $n$ will copy the \emph{execution table} of PIM unit $m$ to its own \emph{execution table} (line 28).
If all tasks in the first level are completed, it can also steal tasks from the second level, and so on.


% \vspace{-0.05in}
\paragraph{Update Schedule Table (lines 30-39)}
Updating \emph{schedule tables} is similar to updating \emph{execution table}. The PIM unit first scans \emph{schedule tables} from the last level to the first level (line 31).
When the first non-null item $T_{sch}$[\emph{i}] is found, it updates the item (lines 32-36). 
If this item is not in the last level, the items in the next level needs to be initialized (lines 37-38).

% Finally the program executes tasks according to \emph{execution table} (Line 11).

% \paragraph{Execute Execution Table (lines 40-47)}
% First, we will introduce the meaning of the index in the table.
% $T_{exe}[i]$ represents the index at level $i$ in the \emph{execution table} of PIM unit $n$.
% The correspondence between $v_0$, $v_1$ and $v_2$ in Figure \ref{fig:AutoMine} and the index in tables is
% $v_0 = T_{exe}[0], v_1 = N(v_0)[T_{exe}[1]], v_2 = N(v_1)[T_{exe}[2]]$, and so on.
% Because when scheduling, the program does not know the length of each neighbor list, if the index of the \emph{execution table} exceeds the length of the neighbor list (line 41), such as $T_{exe}[1]$ exceeds the length of $N(v_0)$, then the program will update \emph{schedule tables} from bottom to top (lines 42-45), otherwise the PIM unit will execute the task according to the index in \emph{execution table} (line 47).
% If the current task does not exist (Line 44), such as $T_{exe}[1]$ exceeds the length of $N(v_0),$ then the program will update \emph{schedule tables} from bottom to top (Lines 45-48).

% \paragraph{Overhead}
% As shown in Figure \ref{fig:PIMMiner}, the \emph{execution table} and \emph{schedule table} of each PIM unit are stored in its nearby bank.
% Based on Algorithm \ref{alg:Stealing}, except for the stealing function, all other operations are performed on their local tables, and these reads and writes are accessed in the same bank group.
% Since PIM has low latency and high bandwidth for memory accesses in the same bank bank group, the overhead of these memory accesses is low.
% For the stealing function, when PIM unit $n$ triggers the stealing mechanism, it will send a request to read \emph{schedule table} to all PIM units.
% After receiving the tables, PIM unit $n$ will choose the unit $m$ to be stolen, update the \emph{schedule table} of unit $m$, and read \emph{execution table} of unit $m$. 
% In this way, the time spent for each stealing is about two times of the memory access latency across channels.
% The size of each \emph{schedule table} is $S \times sizeof(int)$, so each stealing will add $S \times sizeof(int) \times (N_{pim}+2)$ bytes memory access.

%\cb{
% At first, we initialize the \emph{schedule table} of each PIM unit (Line2).
% To increase near bank access, we select the vertex $v$ whose neighbor list $n(v)$ stored in the same bank group with PIM unit as $v_0$ in $Level 0$.
% According to the mapping method in Section \ref{subsec:Local-First Data Mapping}, the neighbor list $N(v)$ of $v=i,i+N_{pim},i+2*N_{pim},...$ is stored on PIM unit $i$, so we use $v_0 = i$ (Lines 12,13) to initialize \emph{schedule table}, and add 128 when updating $v_0$ (Lines 30,39).
% During program execution, the PIM unit first updates \emph{execution table} according to the \emph{schedule table} (Line 4).
% When updating \emph{execution table}, the program first scans \emph{schedule table} from the lowest level to the upper level (Line 15).
% When the first non-null item $T_{sch}$[\emph{i}] is encountered, copy $T_{sch}$[\emph{i}] to $T_{exe}$[\emph{i}] (Lines 16-18).
% However, after updating, if \emph{execution table} $T_{exe}$ is empty (Line 5), which means currently there is no task to execute, then PIM unit $n$ will try to steal some pending tasks from the \emph{schedule table} of other PIM units (Line 6).
% Unlike updating table, stealing will scan the \emph{schedule table} of other PIM units starting from the top level.
% When stealing is triggered, PIM unit $n$ first sends a read request of \emph{execution table} to all PIM units (Line 22).
% Then PIM units scan all \emph{schedule table} from the first level (Line 23).
% In each level, PIM unit prioritizes task whose neighbor list is stored on nearby banks (Line 24).
% After finding the task $j$ to be stolen (Line 25), copy task $j$ to its own \emph{schedule table} $n.T_{sch}$ (Line 26), and send the updated table $j.T_{sch}$ to PIM unit $j$ (Lines 27-30). 
% At the same time, to ensure the correctness of task index at the upper level, PIM unit $n$ will copy the \emph{execution table} of PIM unit $j$ to its own \emph{execution table} (Line 31).
% If all the tasks in the first level are completed, then steal the tasks in the second level, and so on.
% Stealing from the first level is because the task in the first level is large.
% If all tasks are executing, then all \emph{schedule tables} are empty and PIM unit $n$ cannot steal tasks.
% In this case, we consider that the tasks of PIM unit $n$ have all finished, and end the process of PIM unit $n$ (Lines 7,8).
% If \emph{execution table} is not empty, then the PIM unit does not need to steal tasks from other PIM units.
% It will first update \emph{schedule tables}, then execute \emph{execution table} (Lines 10,11).
% Updating \emph{schedule tables} is similar to updating \emph{execution table}, first scan \emph{schedule tables} from the lowest level to the upper level (Line 34).
% When the first non-null item $T_{sch}$[\emph{i}] is encountered, update the item (Lines 35-39). 
% If this item is not in the bottom level, then the item in the next level needs to be initialized (Line 40-41).
% Finally the program executes tasks according to \emph{execution table} (Line 11).
% Reminder, in the table we store the index of each neighbor list, $v_0 = T_{exe}[0], v_1 = N(v_0)[T_{sch}[1]], v_2 = N(v_1)[T_{sch}[2]]$, and so on.
% If the current task does not exist (Line 44), such as $T_{sch}[1]$ exceeds the length of $N(v_0),$ then the program will update \emph{schedule tables} from bottom to top (Lines 45-48).
%}




\begin{algorithm}[t]
\caption{Workload Scheduler with Stealing in PIM Unit $n$}
\label{alg:Stealing}
\small
\begin{algorithmic}[]
\State{\textbf{Input:} \emph{Execution Table $T_{exe}$}, \emph{Schedule Table $T_{sch}$}, \emph{pattern size S}, \emph{PIM unit number} $N_{pim}$; }
\State{e.g., $n.T_{exe}[i]$ is the level $i$ of execution table for PIM unit $n$}

\end{algorithmic}
\hline
\vspace{0.05in}

\begin{algorithmic}[1]
% \State{\textbf{Output}: \emph{border vertex $v_b$}}
%\State{Initialize \emph{Schedule Table $n.T_{sch}$}}
\State \Call{init\_\emph{schedule\_tab}}{}

\While{true}
%\State{Update \emph{Execution Table $n.T_{exe}$} from \emph{Schedule Table $n.T_{sch}$}}
\State \Call{update\_\emph{execution\_tab} }{}
\If{$n.T_{exe}$ is \emph{NULL}}
\State \Call{steal\_\emph{schedule\_tab}}{}
%\State{Steal \emph{Schedule Table $n.T_{sch}$}}
\If{$n.T_{sch}$ is \emph{NULL}}
\State{break}
\EndIf
\Else{}
%\State{Update \emph{Schedule Table $n.T_{sch}$}}
%\State{Execute \emph{Execution Table $n.T_{exe}$}}
\State{\Call{update\_\emph{schedule\_tab}}{}}
\State{\Call{execute\_\emph{execution\_tab}}{}}
\EndIf
\EndWhile
% \State{}
\vspace{0.1in}

\Function{init\_\emph{schedule\_tab}}{}
\State{$n.T_{sch}$[0] $\gets$ $n$}
\EndFunction
% \State{}

\Function{update\_\emph{execution\_tab }}{}
\For{\emph{i} = \emph{S} - 1 \textbf{to} 0}
\State{$n.T_{exe}$[\emph{i}] $\gets$ $n.T_{sch}$[\emph{i}]}
\If{$n.T_{sch}$[\emph{i}] is not \emph{NULL}}
% \State{$n.T_{exe}$[\emph{i}] $\gets$ $n.T_{sch}$[\emph{i}]}
\State{break}
% \Else{}
% \State{$n.T_{exe}$[\emph{i}] $\gets$ \emph{NULL}}
\EndIf
\EndFor
\EndFunction
% \State{}
 
 
 
\Function{steal\_\emph{schedule\_tab}}{}
\State{Get $T_{sch}$ for all PIM Units}
\For{\emph{i} = 0 \textbf{to} \emph{S} - 1}
\State{Select the non-empty $m.T_{sch}$[\emph{i}] of other PIM unit \emph{m}}
% \Comment{(Preferentially select $j.T_{sch}$[\emph{i}] where the neighbor list exists in the bank near PIM unit $n$.)}
\If{\emph{m} exists}
\State{$n.T_{sch}$[\emph{i}] $\gets$ $m.T_{sch}$[\emph{i}]}
\If{\emph{i} = 0}
\State{$m.T_{sch}$[\emph{i}] $\gets$ $m.T_{sch}$[\emph{i}] + $N_{pim}$}
\Else{}
\State{$m.T_{sch}$[\emph{i}] $\gets$ $m.T_{sch}$[\emph{i}] + 1}
\EndIf
% \State{$j.T_{sch}$[\emph{i}] $\gets$ $j.T_{sch}$[\emph{i}] + 1}
\State{$n.T_{exe}$[0:\emph{i-1}] $\gets$ $m.T_{exe}$[0:\emph{i-1}]}
\State{break}
\EndIf
\EndFor
\EndFunction


\Function{update\_\emph{schedule\_tab}}{}
\For{\emph{i} = \emph{S} - 1 \textbf{to} 0}
\If{$n.T_{sch}$[\emph{i}] is not \emph{NULL}}
\If{\emph{i} = 0}
\State{$n.T_{sch}$[\emph{i}] $\gets$ $n.T_{sch}$[\emph{i}] + $N_{pim}$}
\Else{}
\State{$n.T_{sch}$[\emph{i}] $\gets$ $n.T_{sch}$[\emph{i}] + 1}
\EndIf
\If{\emph{i} $<$ \emph{S} - 1}
\State{$n.T_{sch}$[\emph{i}+1] $\gets$ 0}
\EndIf
\State{break}
\EndIf
\EndFor
\EndFunction

\Function{execute\_\emph{execution\_tab}}{}
\If{$n.T_{exe}$ exceeds $len(N(v))$}
\For{\emph{i} = \emph{S} - 1 \textbf{to} 0}
\State{$n.T_{sch}$[\emph{i}] $\gets$ \emph{NULL}}
\If{$n.T_{exe}$[\emph{i}] is not \emph{NULL}}
\State{break}
\EndIf
\EndFor
\Else{}
\State{PIM unit $n$ executes $n.T_{exe}$}
\EndIf
\EndFunction

\end{algorithmic}
\end{algorithm}


% \vspace{-0.05in}
\paragraph{Execute Execution Table (lines 40-47)}
%First, we will introduce the meaning of the index in the table.
% $n.T_{exe}[i]$ stores the index at level $i$ in the \emph{execution table} of PIM unit $n$.
% The correspondence between $v_0$, $v_1$ and $v_2$ in Figure \ref{fig:AutoMine} and the index in tables is
% $v_0 = T_{exe}[0], v_1 = N(v_0)[T_{exe}[1]], v_2 = N(v_1)[T_{exe}[2]]$, and so on.
During the scheduling time, the program does not know the length of each neighbor list.
Therefore, if the index of the \emph{execution table} exceeds the length of the neighbor list (line 41), such as $T_{exe}[1]$ exceeds the length of $N(v_0)$, the program will set \emph{NULL} to \emph{schedule table} from the last level to the first non-null level (lines 42-45). Otherwise the PIM unit will continue executing the task based on the index in \emph{execution table} (line 47).

% \vspace{-0.05in}
\paragraph{Overhead}
As shown in Figure \ref{fig:PIMMiner}, the \emph{execution table} and \emph{schedule table} of each PIM unit are stored in its nearby bank.
Based on Algorithm \ref{alg:Stealing}, except for the stealing function, all other operations are performed on their local tables, and these reads and writes are accessed in their near-core banks.
% the same bank group
Since PIM has low latency and high bandwidth for the near-core bank accesses, the overhead is low.
For the stealing function, when PIM unit $n$ triggers the stealing mechanism, it will send a request to read \emph{schedule table} to all PIM units.
After receiving the tables, PIM unit $n$ will choose the unit $m$ to be stolen, update the \emph{schedule table} of unit $m$, and read \emph{execution table} of unit $m$. 
In this way, the time spent for each stealing is about two times of inter-channel bank access latency.
% the memory access latency across channels.
The size of each \emph{schedule table} is $S \times sizeof(int)$, so each stealing will add $S \times sizeof(int) \times (N_{pim}+2)$ bytes memory access.
% \cb{
In addition, to ensure the consistency of \emph{Schedule Table} $T_{sch}$, when algorithm \ref{alg:Stealing} is executed, it is necessary to ensure that function STEAL\_\emph{SCHEDULE\_TAB} and other functions are mutually exclusive, that is, when function STEAL\_\emph{SCHEDULE\_TAB} is executed, other PIM units need to wait until function STEAL\_\emph{SCHEDULE\_TAB} is completed.
% }

% \begin{figure}[!h]
% \centering 
% \includegraphics[width=\linewidth]{pic/stealingv4.pdf}
% \vspace{-0.3cm}
% \caption{PIM-aware Workload Stealing.} 
% \label{fig:stealing}
% \vspace{-0.2cm}
% \end{figure}



\subsection{Working with GPMI hardware accelerator}
While PIMMiner does not include specialized hardware accelerator unit for GPMI applications, it can cohesively work with proposed accelerator designs \cite{yao2020locality,chen2021flexminer,dai2022dimmining,talati2022ndminer} for the the I/S set operations. By replacing the general-purpose cores with accelerators, we can further improve the performance.
In section \ref{subsec: overall performance}, we evaluate PIMMiner-set, which incorporates the set operation accelerator of FlexMiner\cite{chen2021flexminer} into PIMMiner.




==> section/5_Implementation.tex <==

\subsection{Overview}

hardware diagram

\textbf{HMB-PIM Memory Controller (1).}
HBM-PIM Memory Controller provides a way for CPU to access and manipulate HBM-PIM memory.
In our framework, HBM-PIM Memory Controller provides three basic interface, namely \emph{PIM\_malloc} and \emph{PIM\_free} (2) for allocating space to the specified PIM bank; \emph{CopyToPIM} and \emph{CopyFromPIM} (3) for transferring data between CPU memory and HBM-PIM memory; \emph{PIMReadFile} and \emph{PIMWriteFile} (4) for reading and writing files directly from HBM-PIM memory.
The detail of the interfaces is shown in \S \ref{subsec:interface}.

\subsection{Interface}
\label{subsec:interface}

\subsubsection{CPU-PIM interface}

\subsubsection{PIM-PIM interface}

\subsubsection{GPMI interface}

Preprocessing LoadGraph(G) (include duplication and mapping)

\subsection{Design of Conditional Access Filter}

In our PIMMiner framework, to reduce the interference of memory access filter on PIM units, we add lightweight hardware dedicated to filter unnecessary data on PIM units, as shown in Figure~\ref{fig:PIMMiner} (gray part).
Our conditional filter is designed to handle the memory accesses with bounded data.
The detail of our conditional access filter is shown in Figure~\ref{fig:Filter}.
One 32-bit filter contains one subtractor, one filter logic, and two registers.
When the bank receives a memory access request to the neighbor list $N(v)$, if there are restrictions in memory request, the bank will extract the threshold $th$ and the comparison parameter $cmp$ from the memory request and store them in the two registers (dark blue squares in Figure~\ref{fig:Filter}) respectively.
Then, the filter reads the data $v_x$ from sense amplifier.
$v_x$ is first sent to the subtractor and subtracted with $th$ ($v_x-th$).
The result (1 is positive, 0 is equal, -1 is negative) will be sent to filter logic.
In filter logic, if the result matches the condition $cmp$, output data $v_x$; otherwise, filter out the data.
In this way, only two clock cycles of latency are required for each data filter (one cycle for subtraction, one cycle for comparison).
In our experiment, the width of TSVs on PIM is 64 bits.
Since one filter can handle a 32-bit integer, to maximize TSV bandwidth utilization, we add two filters per bank, which can send 64-bit data per clock cycle.
%Therefore, we place two filters per PIM unit.

\begin{figure}[t]
\centering 
\includegraphics[width=0.4\textwidth]{pic/PIMMiner_Filter.pdf}
\vspace{-0.3cm}
\caption{Conditional access filter.} 
\label{fig:Filter}
\vspace{-0.5cm}
\end{figure}


% \cb{
We assume that the data transferred between PIM units is organized as a packet, which is described in HMC specifications\cite{hmc2013hybrid}. 
A packet without data has 128 bits metadata, which is much smaller than the packet with data (128 bits + 64 Byte Data). In this design, if the data is filtered out, a packet without data is sent to the destination PIM unit; otherwise a packet containing the data pointed to by the address is sent.
% }
% \cb{
We add one bit in the memory request packet to distinguish whether the data is obtained directly or obtained through a filter, thereby helping the memory controller to obtain the data. If the filter is used, the memory request packet will also contain a threshold value and the comparison symbol (we use the less than sign here), and the filter will read vertex IDs according to the address for comparison. If the data is filtered out, we will respond with a packet with no data, otherwise respond with a packet containing the data in this address.
% }


Note that the conditional access filter design can be applied to other workloads that has comparisons, such as database selection operator\cite{kepe2019database}.




\subsection{Design of Local-First Data Mapping}



\subsection{Design of Critical Data Duplication}



\subsection{Design of Workload Stealing}




==> section/6_1_Overall_Performance.tex <==
\subsection{Overall Performance}
\label{subsec: overall performance}
% \hl{add figures for all applications.}

\begin{figure*}[!h]
%\vspace{-0.1in}
\centering 
\includegraphics[width=\linewidth]{pic/Summary1v2.pdf}
\includegraphics[width=\linewidth]{pic/Summary2v2.pdf} 
\includegraphics[width=\linewidth]{pic/Summary3v2.pdf} 
 % \vspace{-0.15in}
\caption{Performance of PIMMiner with the effectiveness of proposed optimizations. In each bar, we show the average time across cores (the solid line) and the total execution time(top of bar).} 
\label{fig:performance}
 \vspace{-0.2in}
\end{figure*}



In this section, we report the overall performance of PIMMiner. 
First, we show the impact of our PIMMiner optimizations on performance.
Then, we compare and report the performance of PIMMiner to other GPMI systems. 


\subsubsection{The performance improvement from PIMMiner optimizations}

Figure \ref{fig:performance} shows the performance improvement of PIMMiner by enabling the five optimizations  proposed in Section \ref{sec:PIMMiner Design} one by one.
In Figure \ref{fig:performance}, the top of bar represents the overall execution time, the solid line represents average execution time for all PIM units.
The difference between the two indicates how imbalanced the workload is.
As shown in Figure \ref{fig:performance}, each of our optimizations reduces the execution time by a fraction; both filter and stealing can help balance workloads across cores.
Conditional access filter achieves 2.01x average speedup and 17.57x maximum speedup over our baseline PIM. 
Local-first data mapping achieves 1.39x average speedup and 2.74x maximum speedup over the filter optimization.
Critical data duplication achieves 1.84x average speedup and 3.05x maximum speedup over our mapping scheme.
The workload scheduler with stealing achieves 3.01x average speedup and 26.87x maximum speedup over the duplication optimization.
And set operation accelerator achieves 1.49x average speedup and 2.26x maximum speedup over the workload scheduler with stealing.
Overall, by enabling all optimizations, \emph{PIMMiner} achieves 12.74x average speedup and 113.76x maximum speedup over the baseline PIM, and \emph{PIMMiner-Set} achieves 15.91x average speedup and 137.32x maximum speedup over the baseline PIM.


In Figure \ref{fig:performance}, the execution time of 4CL-MI and 4DI-YT increases after using local-first data mapping.
The reason is that local-first data mapping increases the possibility of different PIM units accessing the same bank at the same time (for example, all units access N(0) on bank 0 at the same time), resulting in memory access congestion on a few banks.
After remap, 4CL-MI and 4DI-YT access the memory on bank 0 by 3 times and 18 times respectively, and the latency of sending each memory request to the corresponding memory controller also increases by 2-3 times.
The overhead of memory access congestion on a few banks offsets the performance improvement brought by the low latency and high bandwidth of in-bank memory access, resulting in a situation where the execution time increases after using local-first data mapping.
But this memory access congestion can be solved by data duplication.
By copying critical data to each bank, PIM units access their own bank in most cases, so the possibility of PIM units accessing the same memory bank at the same time can be reduced, and the access congestion on a few banks can be alleviated, which is consistent with the results in Figure \ref{fig:performance}.
% We will discuss it in detail in Section \ref{subsec: Benefit Of Our Design}.


% \hl{check the speedup numbers}
% \cb{
% In Figure \ref{fig:performance}, the top of bar represents the overall execution time, the solid line represents average execution time for all PIM units.
% The difference between the two indicates how imbalanced the workload is.
% We can find that both filtering and stealing can reduce part of imbalance problem.
% }




\subsubsection{Compare with other GPMI systems}
% \hl{focus }

Next, we compare our PIMMiner with other GPMI systems, and the results are shown in Table \ref{tab:Graph Mining Systems Comparison}.
In Table \ref{tab:Graph Mining Systems Comparison}, the shortest execution time for each task is in bold, and we can observe that our PIMMiner is the fastest in most cases.
% \cb{
If not the fastest, our PIMMiner is also in the same order of magnitude as the fastest execution time.



In Table \ref{tab:Graph Mining Systems Comparison}, we divide the GPMI systems into 3 types according to their optimization strategies.
The first one is software GPMI system, and the result is obtained by using 96 threads on CPUs.
The second is hardware acceleration, and the result is directly taken from the corresponding paper.
The third one is our proposed PIMMiner and PIMMiner with the specialized set operation accelerator.
% We use Set Intersection/Difference Unit in FlexMiner to accelerate our PIMMiner, which requires one clock cycle for one set operation.
% }

% \cb{
First, we will compare our PIMMiner with the software GPMI systems.
% }
We show the performance of original Automine and our optimized Automine system -- our optimized Automine is faster than GraphPi, except for a few cases.
Our PIMMiner is optimized based on the AutoMine algorithm, and in all applications, PIMMiner is faster than AutoMine.
% For a very few applications, when AutoMine is slower than the other systems or accelerators, our PIMMiner system also takes a slightly longer time to execute, such as 3-MC, 4-CL and 4-DI in several graphs.
% \cb{
On average, our PIMMiner achieves 344x speedup over GraphPi, and 109x speedup over optimized AutoMine.
% }

% \cb{
Then, we will compare our PIMMiner with the hardware GPMI accelerators.
Because these accelerators are optimized for set operations, we also use the PIMMiner with the specialized set operation accelerator (\emph{PIMMiner-Set}) for comparison.
Our \emph{PIMMiner-Set} achieves 696x average speedup over Gramer, 5.9x speedup over FlexMiner, 1.3x speedup over DIMMining, and 37x speedup over NDMiner.
According to the result in Table \ref{tab:Graph Mining Systems Comparison}, the execution time of DIMMining and our PIMMiner is close.
This is because DIMMining uses the Flexible BCSR format to store graphs, so that all graphs can be replicated on each sub-rank, which reduces data transfer time.
In addition, the computing power of DIMMining is much higher than that of PIMMiner. According to the DIMMining paper, DIMMining is running on DRAM at 1.2GHz,
% each DRAM has 32 NMCs, each NMC has 64 PEs, 8 FUs and 32 CUs, 
but our PIMMiner frequency is only 1/5 of DIMMining (250MHz).
Although our PIMMiner has data transfer overhead and low computation frequency, our \emph{PIMMiner-Set} is on the same order of magnitude as DIMMining.
% }


% On average, our PIMMiner achieves 437x speedup over Gramer, 1026x speedup over GraphPi, 166x speedup over FlexMiner, and 837x speedup over optimized AutoMine.
% IntersectX outperforms Gramer by 32x, 85.5x, 121.3x for 3-CC 4-CC and 5-CC respectively.
% Our PIMMiner achieves 3646x, 2990x, 3210x average speedup over Gramer, which is 30 to 100 times faster than IntersectX.
% We believe that an optimized GPMI algorithm could bring more performance improvement room, and our PIMMiner is general and can help achieve better performance by efficiently using PIM architecture. 

% \hl{Compared with DIMMining} why they are so fast


% \begin{table}[!h]
% 	\centering  % 显示位置为中间
% 	\small
% 	%\vspace{-0.1in}
% 	\caption{Graph Mining Systems Comparison (in seconds)}  % 表格标题
% 	\label{tab:Graph Mining Systems Comparison}  % 用于索引表格的标签
% 	%字母的个数对应列数，|代表分割线
% 	% l代表左对齐，c代表居中，r代表右对齐
% 	\vspace{-0.1in}
% 	\resizebox{\linewidth}{!}{
% 	\begin{tabular}{c|c|c|c|c|c|c}  
% 	\hline
% 	    Pattern & Graph & Gramer & GraphPi & FlexMiner & AutoMine (OPT) & PIMMiner\\
% 		\hline  % 表格的横线
% 		\multirow{7}{*}{3-CC} & CI & 9.90E-03 & 4.64E-02 & -- & 4.27E-04 & \textbf{5.30E-06}\\
% 		& PP & 1.00E-02 & 6.72E-02 & -- & 3.77E-03 & \textbf{3.36E-05} \\
% 		& AS & 2.80E-02 & 7.43E-02 & 8.00E-04 & 4.48E-02 & \textbf{2.22E-04}\\
% 		& MI & 1.10E-01 & 9.93E-02 & \textbf{3.7E-04} & 1.24E-01 & 1.46E-03\\
% 		& YT & 13.01 & 2.32E-01 & 2.98E-01 & 9.82E-02 & \textbf{1.21E-02}\\
% 		& PA & 3.09 & 2.32E-01 & 1.25E-01 & 2.11E-01 & \textbf{3.35E-02}\\
% 		& LJ & 17.81 & 2.32 & 3.35E-01 & 6.69E-01 & \textbf{1.59E-01}\\
% 		\hline
% 		\multirow{7}{*}{4-CC} & CI & 1.00E-02 & 5.03E-02 & -- & 4.36E-04 & \textbf{5.86E-06}\\
% 		& PP & 1.10E-02 & 5.14E-02 & -- & 3.79E-03 & \textbf{3.38E-05}\\
% 		& AS & 2.70E-01 & 9.77E-02 & 3.30E-03 & 8.06E-02 & \textbf{7.86E-04}\\
% 		& MI & 6.86 & 4.28E-01 & 5.48E-02 & 2.39E-01 & \textbf{2.77E-02}\\
% 		& YT & 17.3 & 4.83E-01 & 5.14E-01 & 2.08E-01 & \textbf{7.48E-02}\\
% 		& PA & 3.74 & 2.61E-01 & 1.51E-01 & 2.40E-01 & \textbf{3.47E-02}\\
% 		& LJ & 30.89 & 10.58 & -- & 2.78 & \textbf{9.44E-01}\\
% 		\hline
% 		\multirow{7}{*}{5-CC} & CI & 1.10E-02 & 8.19E-02 & -- & 4.70E-04 & \textbf{6.02E-06}\\
% 		& PP & 1.20E-02 & 4.84E-02 & -- & 3.79E-03 & \textbf{3.39E-05}\\
% 		& AS & 1.46 & 1.74E-01 & 2.23E-02 & 1.60E-01 & \textbf{4.68E-03} \\
% 		& MI & 270.41 & 13.89 & -- & 4.35 & \textbf{7.47E-01}\\
% 		& YT & 24.27 & 8.86E-01 & -- & 3.12E-01 & \textbf{2.24E-01}\\
% 		& PA & 4.06 & 3.08E-01 &  8.43E-01 & 1.90E-01 & \textbf{1.62E-02}\\
% 		& LJ & \textbf{52.89} & 291.54 & -- & 99.64 & 95.10\\
% 		\hline
% 		\multirow{7}{*}{3-MC} & CI & 3.10E-02 & 8.88E-02 & -- & 1.25E-03 & \textbf{1.75E-05} \\
% 		& PP & 3.30E-02 & 1.31E-01 & -- & 1.47E-02 & \textbf{1.06E-04}\\
% 		& AS & 1.10E-01 & 1.06E-01 & 1.80E-03 & 7.66E-02 & \textbf{7.97E-04}\\
% 		& MI & 3.60E-01 & 1.63E-01 & 1.29E-02 & 1.89E-01 & \textbf{6.07E-03}\\
% 		& YT & 16.25 & \textbf{4.76E-01} & 8.76E-01 & 1.23 & 6.26E-01\\
% 		& PA & 4.17 & 7.75E-01 & 3.70E-01 & 5.63E-01 & \textbf{1.16E-01} \\
% 		& LJ & 29.68 & 2.77 & -- & 2.37 & \textbf{8.61E-01}\\
% 		\hline
% 		\multirow{7}{*}{4-CY} & CI & -- &  &  & 9.39E-03 & 1.64E-05 \\
% 		& PP & -- &  & -- & 1.03E-02 & 3.03E-04 \\
% 		& AS & -- &  & -- & 3.26E-02 & 7.19E-03 \\
% 		& MI & -- &  & -- & 2.18E-01 & \\
% 		& YT & -- &  & -- & 2.54 & \\
% 		& PA & -- &  & -- & 7.67E-01 &  \\
% 		& LJ & -- &  & -- & 40.09 & \\
% 		\hline
% 		\multirow{7}{*}{4-DI} & CI & -- &  &  & 9.50E-03 & 1.97E-05 \\
% 		& PP & -- &  & -- & 1.13E-02 & 3.67E-04 \\
% 		& AS & -- &  & -- & 4.25E-02 & 9.26E-03\\
% 		& MI & -- &  & -- & 0.394951 & \\
% 		& YT & -- &  & -- & 2.79875 & \\
% 		& PA & -- &  & -- & 1.15982 &  \\
% 		& LJ & -- &  & -- & 65.2918 & \\
% 		\hline
% 	\end{tabular}
% 	}
% \end{table}






\begin{table*}[t]
	\centering  % 显示位置为中间
	\small
	%\vspace{-0.1in}
	\caption{Graph Mining Systems Comparison (in seconds)\\ AM is the abbreviation of AutoMine. In the DIM\&ND column, graphs PP, AS, MI are the results of DIMMining, and graph PA is the result of NDMiner.}  % 表格标题
	\label{tab:Graph Mining Systems Comparison}  % 用于索引表格的标签
	%字母的个数对应列数，|代表分割线
	% l代表左对齐，c代表居中，r代表右对齐
	% \vspace{-0.1in}
	\resizebox{0.75\linewidth}{!}{
	\begin{tabular}{c|c|c|c|c|c|c|c|c}  
	\hline
	    Pattern & GPMI & CI & PP & AS & MI & YT & PA & LJ\\
		\hline  % 表格的横线
		\multirow{9}{*}{3-CC} 
		& GraphPi & 4.64E-02 & 6.72E-02 & 7.43E-02 & 9.93E-02 & 2.32E-01 & 2.32E-01 & 2.32 \\
		& AutoMine (ORG) & 1.45E-02 & 3.57E-02 & 3.22E-01 & 2.53 & 23.39 & 21.84  & 186.61 \\
		& AutoMine (OPT) & 4.87E-03 & 9.54E-03 & 1.12E-02 & 2.69E-02 & 1.34E-01 & 1.98E-01 & 1.24 \\ 
		\cline{2-9}
		& Gramer & 9.90E-03 & 1.00E-02 & 2.80E-02 & 1.10E-01 & 13.01 & 3.09 & 17.81\\
		& FlexMiner & -- &-- & 5.00E-04 & 2.30E-03 & 1.86E-01 & 7.84E-02 & 2.10E-01\\
        & DIMMining & -- & 1.59E-05 & 2.56E-04 & 1.57E-03 & 1.16E-02 & \textbf{1.48E-02} & \textbf{6.90E-02} \\ 
        & NDMiner & -- & -- & -- & -- & -- & 2.30E-01 & 7.36E-01 \\ 
        \cline{2-9}
		& PIMMiner & 5.30E-06 & 3.36E-05 & 2.22E-04 & 1.46E-03 & 1.21E-02 & 3.35E-02 & 1.59E-01\\
        & PIMMiner-Set & \textbf{3.09E-06} & \textbf{1.51E-05} & \textbf{1.49E-04} & \textbf{1.03E-03} & \textbf{1.10E-02} & 1.52E-02 & 1.22E-01 \\ 
	\hline
		\multirow{9}{*}{4-CC} 
            & GraphPi & 1.49E-02 & 1.23E-02 & 1.91E-02 & 2.37E-01 & 2.01E-01 & 2.94E-01 & 6.53 \\
            & AutoMine (ORG) & 1.07E-03 & 1.00E-02 & 6.29E-01 & 11.82 & 3.05 & 3.47  &  256.42 \\
            & AutoMine (OPT) & 4.36E-04 & 3.79E-03 & 8.06E-02 & 2.39E-01 & 2.08E-01 & 2.40E-01 & 2.78 \\ 
            \cline{2-9}
            & Gramer & 1.00E-02 & 1.10E-02 & 2.70E-01 & 6.86 & 17.3 & 3.74 & 30.89\\
		& FlexMiner & -- &-- & 2.10E-03 & 3.43E-02 & 3.21E-01 & 9.46E-02 & --\\
            & DIMMining & -- & 1.71E-05 & 1.58E-03 & \textbf{2.22E-02} & \textbf{1.54E-02} & 1.80E-02 & \textbf{4.38E-01} \\ 
            & NDMiner & -- & -- & -- & -- & -- & 4.61E-01 & 14.08 \\ 
            \cline{2-9}
		& PIMMiner & 5.86E-06 & 3.38E-05 & 7.86E-04 & 2.77E-02 & 7.84E-02 & 3.47E-02 & 1.16 \\
            & PIMMiner-Set & \textbf{3.43E-06} & \textbf{1.52E-05} & \textbf{6.51E-04} & 2.49E-02 & 6.57E-02 & \textbf{1.74E-02 }&  9.61E-01\\ 
	\hline
	    \multirow{9}{*}{5-CC} 
            & GraphPi & 1.62E-02 & 1.22E-02 & 6.10E-02 & 10.36  & 4.53E-01 & 1.61E-01 & 210.01 \\
            & AutoMine (ORG) & 2.08E-03 & 8.81E-03 & 6.31  & 2110.88  & 97.94  & 5.17  & 51,473.6 \\
		& AutoMine (OPT) & 4.70E-04 & 3.79E-03 & 1.60E-01 & 4.35 & 3.12E-01 & 1.90E-01 & 99.64 \\ 
             \cline{2-9}
            & Gramer & 1.10E-02 & 1.20E-02 & 1.46 & 270.41 & 24.27 & 4.06 & \text{52.89}\\
		& FlexMiner & -- &-- & 1.39E-02 & -- & -- & 5.27E-01 & --\\
            & DIMMining & -- & 1.72E-05 & 1.01E-02 & 7.76E-01 & 2.88E-02 & 1.94E-02 & \textbf{13.47} \\ 
            & NDMiner & -- & -- & -- & -- & -- & 9.19E-01 & -- \\ 
             \cline{2-9}
		& PIMMiner & 6.02E-06 & 3.39E-05 & 4.68E-03 & 7.47E-01 & 2.24E-01 & 1.62E-02 & 95.10\\
            & PIMMiner-Set & \textbf{3.70E-06} & \textbf{1.53E-05} & \textbf{4.03E-03} & \textbf{6.19E-01} & \textbf{2.19E-01} & \textbf{1.22E-02} & 88.78 \\ 
	\hline
	    \multirow{9}{*}{3-MC} 
            & GraphPi & 1.84E-02 & 2.12E-02 & 3.32E-02 & 3.69E-02 & 2.32E-01 & 2.76E-01 & 1.04 \\
            & AutoMine (ORG) & 1.65E-02 & 4.56E-02 & 4.08E-01 & 3.23  & 25.39  & 27.07  & 218.09  \\
		& AutoMine (OPT) & 1.43E-02 & 1.70E-02 & 1.76E-02 & 4.26E-02 & 4.48E-01 & 3.28E-01 & 1.72  \\ 
            \cline{2-9}
            & Gramer & 3.10E-02 & 3.30E-02 & 1.10E-01 & 3.60E-01 & 16.25 & 4.17 & 29.68\\
		& FlexMiner & -- & -- & 1.10E-03 & 8.10E-03 & 5.47E-01 & 2.31E-01 & --\\
            & DIMMining & -- & 4.74E-05 & 9.08E-04 & 6.18E-03 & \textbf{1.16E-01} & 4.79E-02 & 3.29E-01 \\ 
            & NDMiner & -- & -- & -- & -- & -- & -- & 4.10\\ 
            \cline{2-9}
		& PIMMiner & 1.09E-05 & 4.96E-05 & 3.44E-04 & 3.07E-03 & 1.75E-01 & 4.34E-02 & 3.56E-01\\
            & PIMMiner-Set & \textbf{8.64E-06} & \textbf{2.69E-05} & \textbf{2.60E-04} & \textbf{2.52E-03} & 1.73E-01 & \textbf{2.48E-02} & \textbf{3.14E-01} \\ 
	\hline
	    \multirow{7}{*}{4-CL} 
            & GraphPi  & 1.09E-02 & 1.23E-02 & 3.26E-02 & 4.31E-01 & 2.29   &   4.13E-01 & 31.09 \\
		& AutoMine (ORG) & 2.52E-03 & 2.78E-02 & 3.17E-01 & 3.21  & 18.83  & 28.75  &  417.03 \\
		& AutoMine (OPT) & 1.50E-03 & 1.03E-02 & 3.26E-02 & 2.18E-01 & 2.54 & 7.67E-01 & 40.09 \\ 
            \cline{2-9}
            & NDMiner & -- & -- & -- & -- & -- & 6.04 & -- \\
            \cline{2-9}
		& PIMMiner & 6.54E-06 & 6.60E-05 & 2.99E-03 &  9.19E-02 & 2.80E-01 & 6.24E-02 & 6.01   \\
            & PIMMiner-Set & \textbf{4.56E-06} & \textbf{4.68E-05} &  \textbf{2.60E-03} & \textbf{8.32E-02} & \textbf{2.07E-01} & \textbf{4.78E-02} & \textbf{4.97}  \\ 
	\hline
	\multirow{8}{*}{4-DI} 
        & GraphPi & 1.03E-02 & 1.18E-02 & 1.70E-02 & 7.28E-02 & 9.25E-02 & 1.63E-01 & 1.91 \\
		& AutoMine (ORG) & 2.43E-03 & 1.13E-02 & 1.04 & 25.49  & 8.78  & 11.70  & 705.40  \\
		& AutoMine (OPT) & 9.39E-03 & 9.83E-03 & 1.02E-02 & 2.34E-01 & 1.23E-01 & 1.37E-01 & 5.54 \\ 
        \cline{2-9}
        & FlexMiner & -- & -- & 9.00E-04 & 7.10E-03 & 2.18E-01 & 8.10E-02 & \textbf{3.18E-01}\\
	& DIMMining & -- & \text{3.98E-05} & \textbf{6.19E-04} & \textbf{4.92E-03} & \text{1.28E-01} & \text{3.69E-02} & 3.21E-01 \\ 
        & NDMiner & -- & -- & -- & -- & -- & 5.05E-01 & -- \\
        \cline{2-9}
	& PIMMiner & 7.21E-06 & 4.64E-05 & 1.22E-03 & 3.01E-02 & 8.30E-02 & 4.34E-02 & 1.02 \\
            & PIMMiner-Set & \textbf{4.41E-06} & \textbf{2.93E-05} & \text{1.09E-03} & \text{2.89E-02} & \textbf{6.53E-02} & \textbf{2.97E-02} & \text{9.20E-01} \\ 
	\hline
	\end{tabular}
	}
\end{table*}

























\iffalse
\begin{table}[!h]
	\centering  % 显示位置为中间
	\small
	\vspace{-0.1in}
	\caption{Graph Mining Systems Comparison (/SEC.)}  % 表格标题
	\label{tab:Graph Mining Systems Comparison}  % 用于索引表格的标签
	%字母的个数对应列数，|代表分割线
	% l代表左对齐，c代表居中，r代表右对齐
	\vspace{-0.1in}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{c|c|c|c|c|c|c}  
	\hline
	    Pattern & Graph & Gramer & GraphPi & FlexMiner & AutoMine & PIMMiner\\
		\hline  % 表格的横线
		\multirow{7}{*}{3-CC} & CI & 9.90E-03 & 4.64E-02 &  & 4.27E-04 & \textbf{4.70E-06}\\
		& PP & 1.00E-02 & 6.72E-02 &  & 3.77E-03 & \textbf{3.27E-05} \\
		& AS & 2.80E-02 & 7.43E-02 & 8.00E-04 & 4.48E-02 & \textbf{2.18E-04}\\
		& MI & 1.10E-01 & 9.93E-02 & 3.7E-04 & 1.24E-01 & \textbf{1.41E-03}\\
		& YT & 13.01 & 2.32E-01 & 2.98E-01 & 9.82E-02 & \textbf{1.19E-02}\\
		& PA & 3.09 & 2.32E-01 & 1.25E-01 & 2.11E-01 & \textbf{3.34E-02}\\
		& LJ & 17.81 & 2.32 & 3.35E-01 & 6.69E-01 & \textbf{1.60E-01}\\
		\hline
		\multirow{7}{*}{4-CC} & CI & 1.00E-02 & 5.03E-02 &  & 4.36E-04 & \textbf{5.21E-06}\\
		& PP & 1.10E-02 & 5.14E-02 & & 3.79E-04 & \textbf{3.29E-05}\\
		& AS & 2.70E-01 & 9.77E-02 & 3.30E-03 & 8.06E-02 & \textbf{7.74E-04}\\
		& MI & 6.86 & 4.28E-01 & 5.48E-02 & 2.39E-01 & \textbf{2.74E-02}\\
		& YT & 17.3 & 4.83E-01 & 5.14E-01 & 2.08E-01 & \textbf{7.49E-02}\\
		& PA & 3.74 & 2.61E-01 & 1.51E-01 & 2.40E-01 & \textbf{3.45E-02}\\
		& LJ & 30.89 & 10.58 &  & 2.78 & \textbf{9.32E-01}\\
		\hline
		\multirow{7}{*}{5-CC} & CI & 1.10E-2 & 8.19E-02 &  & 4.70E-04 & \textbf{5.34E-06}\\
		& PP & 1.20E-02 & 4.84E-02 &  & 3.79E-03 & \textbf{3.30E-05}\\
		& AS & 1.46 & 1.74E-01 & 2.23E-02 & 1.60E-01 & \textbf{4.66E-03} \\
		& MI & 270.41 & 13.89 &  & 4.35 & \textbf{7.42E-01}\\
		& YT & 24.27 & 8.86E-01 &  & 3.12E-01 & \textbf{2.24E-01}\\
		& PA & 4.06 & 3.08E-01 &  8.43E-01 & 1.90E-01 & \textbf{1.58E-02}\\
		& LJ & 52.89 & 291.54 &  & 89.64 & \\
		\hline
		\multirow{7}{*}{3-MC} & CI & 3.10E-02 & 8.88E-02 &  & 1.25E-03 & \textbf{1.64E-05} \\
		& PP & 3.30E-02 & 1.31E-01 &  & 1.47E-02 & \textbf{1.03E-04}\\
		& AS & 1.10E-01 & 1.06E-01 & 1.80E-03 & 7.66E-02 & \textbf{7.87E-04}\\
		& MI & 3.60E-01 & 1.63E-01 & 1.29E-02 & 1.89E-01 & \textbf{5.92E-03}\\
		& YT & 16.25 & \textbf{4.76E-01} & 8.76E-01 & 1.23 & 6.25E-01\\
		& PA & 4.17 & 7.75E-01 & 3.70E-01 & 5.63E-01 & \textbf{1.16E-01} \\
		& LJ & 29.68 & 2.77 &  & 2.37 & \textbf{8.68E-01}\\
		\hline
	\end{tabular}
	}
\end{table}
\fi



==> section/6_2_Benefit_of_Design.tex <==
\iffalse
\subsection{In-depth Study}
\label{subsec: Benefit Of Our Design}

% \hl{show this for 4-CC.}
In this section, we will take 4-CC as an example to compare the performance improvement and memory access reduction brought by each optimization. 
% \cb{
Because the specialized set operation accelerator is not proposed by us, due to space limitations, we do not discuss the specialized set operation accelerator in this section.
% }

\subsubsection{Benefit of Conditional Access Filter}

First, we discuss the impact of conditional access filter on memory access.
Table \ref{tab:Benefit Of Conditional Access Filtering} shows the memory access size of 4-CC before and after filtering.
Conditional access filter can reduce the memory footprint by 22\% to 85\%. 
This optimization could significantly enhance performance for graphs that trigger a larger memory footprint. For example, \emph{Astro} is a small graph that has a memory footprint (165.70MB) about 31x over the graph size (5.3MB). Although the graph size is small, conditional access filter can achieve significant speedup by removing 78\% redundant memory accesses.
For other graphs with more than 100 MB of memory footprint, the filter design also reduces memory accesses by more than 60\% and execution time by more than half.

\begin{table}[t]
	\centering  % 显示位置为中间
	\small
	\vspace{-0.1in}
	\caption{Benefit of Conditional Access Filter in 4-CC.}  % 表格标题
	\label{tab:Benefit Of Conditional Access Filtering}  % 用于索引表格的标签
	%字母的个数对应列数，|代表分割线
	% l代表左对齐，c代表居中，r代表右对齐
	% \vspace{-0.1in}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{c|c|c|c|c}  
	\hline
	    Graph & Total & Filtered & Memory Footprint & Exe Time \\
	     & Access & Access & reduction ratio & Speedup \\
		\hline  % 表格的横线
	    CI & 1.30MB & 1.01MB & 22\% & 1.13x \\
		PP & 8.21MB & 5.48MB & 33\% & 1.19x \\
		AS & 165.70MB & 36.85MB & 78\% & 2.76x \\
		MI & 2.10GB & 315.88MB & 85\% & 2.41x \\
		YT & 1.17GB & 474.17MB & 59\% & 2.64x \\
		PA & 48.01MB & 29.99MB & 38\% & 1.30x \\
		LJ & 706.70MB & 143.66MB & 80\% & 2.90x \\
		\hline
	\end{tabular}
	}
 \vspace{-0.2in}
\end{table}

\fi

% \begin{table}[t]
% 	\centering  % 显示位置为中间
% 	\small
% 	\vspace{-0.1in}
% 	\caption{Benefit of Conditional Access Filter in 4-CC.}  % 表格标题
% 	\label{tab:Benefit Of Conditional Access Filtering}  % 用于索引表格的标签
% 	%字母的个数对应列数，|代表分割线
% 	% l代表左对齐，c代表居中，r代表右对齐
% 	\vspace{-0.1in}
% 	\resizebox{0.9\linewidth}{!}{
% 	\begin{tabular}{c|c|c|c|c}  
% 	\hline
% 	    Graph & Total & Filtered & Memory Footprint & Exe Time \\
% 	     & Access & Access & reduction ratio & Speedup \\
% 		\hline  % 表格的横线
% 	    CI & 1.30MB & 1.01MB & 22\% & 1.13x \\
% 		PP & 8.21MB & 5.48MB & 33\% & 1.19x \\
% 		AS & 165.70MB & 36.85MB & 78\% & 2.76x \\
% 		MI & 2.10GB & 315.88MB & 85\% & 2.41x \\
% 		YT & 1.17GB & 474.17MB & 59\% & 2.64x \\
% 		PA & 48.01MB & 29.99MB & 38\% & 1.30x \\
% 		LJ & 706.70MB & 143.66MB & 80\% & 2.90x \\
% 		\hline
% 	\end{tabular}
% 	}
% \end{table}
% \vspace{-0.1in}

% \begin{table}[!h]
% 	\centering  % 显示位置为中间
% 	\small
% 	\vspace{-0.1in}
% 	\caption{Benefit Of Conditional Access Filtering in 3-CC.}  % 表格标题
% 	\label{tab:Benefit Of Conditional Access Filtering}  % 用于索引表格的标签
% 	%字母的个数对应列数，|代表分割线
% 	% l代表左对齐，c代表居中，r代表右对齐
% 	\vspace{-0.1in}
% 	\resizebox{0.9\linewidth}{!}{
% 	\begin{tabular}{c|c|c|c|c}  
% 	\hline
% 	    Graph & Total & Filtered & Memory Footprint & Exe Time \\
% 	     & Access & Access & reduction ratio & Speedup \\
% 		\hline  % 表格的横线
% 	    CI & 1.24MB & 0.96MB & 0.23 & 1.15x \\
% 		PP & 8.13MB & 5.41MB & 0.33 & 1.09x \\
% 		AS & 94.48MB & 35.57MB & 0.62 & 1.55x \\
% 		MI & 64.57MB & 25.38MB & 0.61 & 1.98x \\
% 		YT & 370.23MB & 129.19MB & 0.65 & 2.24x \\
% 		PA & 54.91MB & 32.55MB & 0.41 & 1.22x \\
% 		LJ & 119.00MB & 35.55MB & 0.70 & 2.61x \\
% 		\hline
% 	\end{tabular}
% 	}
% \end{table}

\iffalse

\subsubsection{Benefit of Local-First Data Mapping}

Next, we analyze the benefit of local-first data mapping. We measure the accesses that fall into the local banks, as well as the latency of memory requests.
% \cb{
% In Table \ref{tab:Benefit of Local-First Data Mapping}, in-bank ratio is the ratio of the number of memory accesses in the same bank group to all memory accesses.
% }
% There are two kinds of latency in Table \ref{tab:Benefit of Local-First Data Mapping}.
% Among them, 
Send latency refers to the number of cycles that each memory access request is sent from PIM unit to the corresponding bank, and response latency refers to the number of cycles required for the memory access to return from the bank to the PIM unit.
After remapping, the ratio of local memory accesses increases significantly.
Because of the low latency and high bandwidth of local memory accesses on PIM, the local bank access ratio increases, resulting in lower send latency and response latency, thereby reducing execution time.
In Table \ref{tab:Benefit of Local-First Data Mapping}, after \emph{CiteSeer} and \emph{Youtube} are remapped, the local access ratio is significantly improved, especially for \emph{Youtube}, where the local access ratio reaches 98.62\%, which shows that \emph{Youtube} can achieve good locality of memory access without duplication.
For other graphs, although remapping has only a little improvement in local access ratio and performance, local-first data mapping is the basis for the next duplication optimization.




\begin{table}[!h]
	\centering  % 显示位置为中间
	\small
	\vspace{-0.1in}
	\caption{Benefit of Local-First Data Mapping in 4-CC. (Local access ratio = PIM memory accesses in the local bank group over all memory accesses.)}  % 表格标题
	\label{tab:Benefit of Local-First Data Mapping}  % 用于索引表格的标签
	%字母的个数对应列数，|代表分割线
	% l代表左对齐，c代表居中，r代表右对齐
	% \vspace{-0.1in}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{c|c|c|c|c|c}  
	\hline
	    Graph & Mapping & Local access & Send & Response & Exe Time\\
	     &  & ratio & latency & latency & Speedup \\
		\hline  % 表格的横线
	    \multirow{2}{*}{CI} & Convention & 1.36\% & 5209 & 175 & \multirow{2}{*}{2.74x} \\
	    & Local-First & 86.86\% & 123 & 58 & \\
	    \hline
		\multirow{2}{*}{PP} & Convention & 1.36\% & 1276 & 158 & \multirow{2}{*}{1.33x} \\
		& Local-First & 60.19\% & 93 & 79 & \\
		\hline
		\multirow{2}{*}{AS} & Convention & 1.78\% & 583 & 151 & \multirow{2}{*}{1.03x} \\
		& Local-First & 32.68\% & 124 & 117 & \\
		\hline
		\multirow{2}{*}{MI} & Convention & 2.03\% & 260 & 151 & \multirow{2}{*}{1.01x} \\
		& Local-First & 19.31\% & 194 & 137 & \\
		\hline
		\multirow{2}{*}{YT} & Convention & 1.22\% & 1926 & 140 & \multirow{2}{*}{1.73x} \\
		& Local-First & 98.62\% & 978 & 16 & \\
		\hline
		\multirow{2}{*}{PA} & Convention & 1.33\% & 544 & 153 & \multirow{2}{*}{1.12x} \\
		& Local-First & 50.34\% & 94 & 89 & \\
		\hline
		\multirow{2}{*}{LJ} & Convention & 5.74\% & 513 & 146 & \multirow{2}{*}{1.05x} \\
		& Local-First & 69.23\% & 466 & 59 & \\
		\hline
	\end{tabular}
	}
 \vspace{-0.2in}
\end{table}

\fi


\iffalse
\begin{table}[!h]
	\centering  % 显示位置为中间
	\small
	\vspace{-0.1in}
	\caption{Benefit of Local-First Data Mapping in 3-CC.}  % 表格标题
	\label{tab:Benefit of Local-First Data Mapping}  % 用于索引表格的标签
	%字母的个数对应列数，|代表分割线
	% l代表左对齐，c代表居中，r代表右对齐
	\vspace{-0.1in}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{c|c|c|c|c|c}  
	\hline
	    Graph & Mapping & Local access ratio & Send latency & Response latency & Time Speedup\\
		\hline  % 表格的横线
	    \multirow{2}{*}{CI} & Convention & 1.30\% & 3573 & 173 & \multirow{2}{*}{2.29x} \\
	    & Local-First & 85.84\% & 102 & 61 & \\
	    \hline
		\multirow{2}{*}{PP} & Convention & 1.45\% & 1387 & 156 & \multirow{2}{*}{1.38x} \\
		& Local-First & 59.51\% & 88 & 81 & \\
		\hline
		\multirow{2}{*}{AS} & Convention & 1.29\% & 474 & 153 & \multirow{2}{*}{1.04x} \\
		& Local-First & 30.63\% & 118 & 122 & \\
		\hline
		\multirow{2}{*}{MI} & Convention & 1.33\% & 766 & 156 & \multirow{2}{*}{1.09x} \\
		& Local-First & 37.30\% & 158 & 121 & \\
		\hline
		\multirow{2}{*}{YT} & Convention & 0.99\% & 2216 & 142 & \multirow{2}{*}{2.06x} \\
		& Local-First & 95.25\% & 934 & 21 & \\
		\hline
		\multirow{2}{*}{PA} & Convention & 1.31\% & 500 & 153 & \multirow{2}{*}{1.23x} \\
		& Local-First & 58.71\% & 81 & 78 & \\
		\hline
		\multirow{2}{*}{LJ} & Convention & 1.12\% & 1483 & 147 & \multirow{2}{*}{1.35x} \\
		& Local-First & 76.61\% & 640 & 56 & \\
		\hline
	\end{tabular}
	}
\end{table}
\fi

\iffalse    
\subsubsection{Benefit of Critical Data Duplication}
% \hl{sensitivity study on duplication ratio v.s. speedup for first five graphs.}
Then, we show the improvement of data locality through critical data duplication.
First, according to Algorithm \ref{alg:Critical Data}, we calculate the maximum number of the neighbor list duplication that each bank group can store.
As can be seen from Table \ref{tab:Benefit of Critical Data Duplication}, the first five graphs can duplicate the entire graph in each bank group since they are very small.
The last two graphs are large; therefore, the algorithm selects the top 5\% and 0.25\% neighbor list for duplication and stores them in each bank group.
With data duplication, the local access memory access ratio of the first 5 graphs reaches 100\%, \emph{LiveJournal} also reaches 90\% , and \emph{Patents} reaching 60\%.
The speedup achieved through critical data duplication is significant, even for the larger graphs that cannot fully duplicate the neighbor lists, such as \emph{LiveJournal} and \emph{Patents}.
Note that, in Table \ref{tab:Benefit of Critical Data Duplication}, the request send latency of \emph{Youtube} and \emph{LiveJournal} is slightly increased.
We believe this is because of the imbalanced workload, which leads to excessive memory access pressure on a few bank groups, and thus the memory access latency becomes longer.



\begin{table}[!h]
	\centering  % 显示位置为中间
	\small
	% \vspace{-0.1in}
	\caption{Benefit of Critical Data Duplication in 4-CC.}  % 表格标题
	\label{tab:Benefit of Critical Data Duplication}  % 用于索引表格的标签
	%字母的个数对应列数，|代表分割线
	% l代表左对齐，c代表居中，r代表右对齐
	% \vspace{-0.1in}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{c|c|c|c|c|c}  
	\hline
	    Graph & Duplicate & Local access ratio & Send latency & Response latency & Time Speedup\\
		\hline  % 表格的横线
	    \multirow{2}{*}{CI} & No & 86.86 & 123 & 58 & \multirow{2}{*}{2.12x} \\
	    & Top 100\% & 100.00\% & 108 & 43 & \\
	    \hline
		\multirow{2}{*}{PP} & No & 60.19\% & 93 & 79 & \multirow{2}{*}{3.04x} \\
		& Top 100\% & 100.00\% & 43 & 30 & \\
		\hline
		\multirow{2}{*}{AS} & No & 32.68\% & 124 & 117 & \multirow{2}{*}{1.39x} \\
		& Top 100\% & 100.00\% & 40 & 31 & \\
		\hline
		\multirow{2}{*}{MI} & No & 19.31\% & 194 & 137 & \multirow{2}{*}{1.86x} \\
		& Top 100\% & 100.00\% & 99 & 35 & \\
		\hline
		\multirow{2}{*}{YT} & No & 98.62\% & 978 & 16 & \multirow{2}{*}{1.09x} \\
		& Top 100\% & 100.00\% & 982 & 14 & \\
		\hline
		\multirow{2}{*}{PA} & No & 50.34\% & 94 & 89 & \multirow{2}{*}{1.26x} \\
		& Top 5.33\% & 66.27\% & 75 & 70 & \\
		\hline
		\multirow{2}{*}{LJ} & No & 69.23\% & 466 & 59 & \multirow{2}{*}{1.75x} \\
		& Top 0.25\% & 90.51\% & 552 & 50 & \\
		\hline
	\end{tabular}
	}
 \vspace{-0.2in}
\end{table}



\iffalse
\begin{table}[!h]
	\centering  % 显示位置为中间
	\small
	\vspace{-0.1in}
	\caption{Benefit of Critical Data Duplication in 3-CC.}  % 表格标题
	\label{tab:Benefit of Critical Data Duplication}  % 用于索引表格的标签
	%字母的个数对应列数，|代表分割线
	% l代表左对齐，c代表居中，r代表右对齐
	\vspace{-0.1in}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{c|c|c|c|c|c}  
	\hline
	    Graph & Duplicate & Local access ratio & Send latency & Response latency & Time Speedup\\
		\hline  % 表格的横线
	    \multirow{2}{*}{CI} & No & 85.84\% & 102 & 61 & \multirow{2}{*}{2.27x} \\
	    & Top 100\% & 100.00\% & 86 & 45 & \\
	    \hline
		\multirow{2}{*}{PP} & No & 59.51\% & 88 & 81 & \multirow{2}{*}{3.05x} \\
		& Top 100\% & 100.00\% & 30 & 4.4 & \\
		\hline
		\multirow{2}{*}{AS} & No & 30.63\% & 118 & 122 & \multirow{2}{*}{2.78x} \\
		& Top 100\% & 100.00\% & 30 & 31 & \\
		\hline
		\multirow{2}{*}{MI} & No & 37.30\% & 158 & 121 & \multirow{2}{*}{2.47x} \\
		& Top 100\% & 100.00\% & 79 & 34 & \\
		\hline
		\multirow{2}{*}{YT} & No & 95.25\% & 934 & 21 & \multirow{2}{*}{1.28x} \\
		& Top 100\% & 100.00\% & 928 & 15 & \\
		\hline
		\multirow{2}{*}{PA} & No & 58.71\% & 81 & 78 & \multirow{2}{*}{1.38x} \\
		& Top 5.33\% & 76.07\% & 60 & 57 & \\
		\hline
		\multirow{2}{*}{LJ} & No & 76.61\% & 640 & 56 & \multirow{2}{*}{1.17x} \\
		& Top 0.25\% & 81.14\% & 634 & 50 & \\
		\hline
	\end{tabular}
	}
\end{table}
\fi


We also perform a sensitivity study on the duplication size and speedup for the five smaller graphs.
% \cb{
The duplicated method is shown in Algorithm \ref{alg:Critical Data}, in Figure \ref{fig:dup speedup}, the x-axis is the relative data duplication size ($M=(1+x)G.size$ in Algorithm \ref{alg:Critical Data}), which is calculated as the ratio of critical data size over the input graph size: 1 means that total duplication size is the size of the graph ($M=2 \times G.size$), and 128 means that the total duplication size is 128 times of the graph ($M=129 \times G.size$).
% }
%In Table \ref{tab:Benefit of Critical Data Duplication}, the duplication ratio of each graph is only related to the size of the graph, so the duplication size is related to the graph size.
% In Figure \ref{fig:dup speedup}, the x-axis is the relative data duplication size, which is calculated as the ratio of critical data size over the input graph size: 1 means that total duplication size is the size of the graph, and 128 means that the total duplication size is 128 times of the graph.
%Since we only have 128 PIM units, 128 also means that each bank group stores a graph.
The y-axis is the speedup of the execution time over the execution time without duplication but with filter and remapping.
In Figure \ref{fig:dup speedup}, the overall improvement for graph \emph{Youtube} is small, because the local access ratio of \emph{Youtube} has reached 98.62\% without the duplication, so there is no room for improvement in duplication.
For \emph{Mico} graph, the duplication size from 0 to 16 times, the local access ratio increases from 19\% to 92\%, thus resulting in a faster increase in the first 16-size speedup. After that, since there is no room for growth in the local access ratio, the speedup of \emph{Mico} is basically flat.
For other graphs, the local access ratio increases gradually with the increase of duplication size, and the speedup of execution time also increases linearly.





\begin{figure}[h]
\centering 
\vspace{-0.15in}
\includegraphics[width=0.8\linewidth]{pic/4-CC_dup_speedup.pdf}
\vspace{-0.2cm}
\caption{Speedup - Critical Data Duplication Size Tradeoff in 4-CC ($x$ axis = Critical Data Size / Input Graph Size).} 
\label{fig:dup speedup}
\vspace{-0.1cm}
\end{figure}

\fi


\subsubsection{Benefit of Workload Stealing}
% \hl{just show the execution time/average time ratio}
In Figure \ref{fig:performance}, as the pattern size increases, the gap between the execution time and average time becomes larger, which means that the workload becomes more and more imbalanced.
The conditional access filter reduces load imbalance issues for several applications; for larger patterns, our workload stealing can further mitigate the load imbalance issues dynamically.
We analyze 4-CC in Table \ref{tab:Benefit Of PIM-aware Work Stealing}.
The first row shows the ratio of the execution time to the average time after the first three optimizations.
We can observe that even with the prior optimizations, \emph{Mico}, \emph{Youtube} and \emph{LiveJournal} still have significant load imbalance issues.
With the workload stealing scheme, the difference between execution time and
average time becomes negligible.
Our scheduler with workload stealing on 4-CC can achieve up to 20x speedup.


\begin{table}[!h]
	\centering  % 显示位置为中间
	\small
	%\vspace{-0.1in}
	\caption{Benefit of Workload Stealing in 4-CC.}  % 表格标题
	\label{tab:Benefit Of PIM-aware Work Stealing}  % 用于索引表格的标签
	%字母的个数对应列数，|代表分割线
	% l代表左对齐，c代表居中，r代表右对齐
	%\vspace{-0.1in}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{c|c|c|c|c|c|c|c}  
	\hline
	    Graph & CI & PP & AS & MI & YT & PA & LJ \\
		\hline  % 表格的横线
		Exe/Avg (no steal) & 1.28 & 1.09 & 1.33 & 3.46 & 5.24 & 1.09 & 22.23 \\
		Exe/Avg (steal) & 1.06 & 1.004 & 1.001 & 1.001 & 1.01 & 1.001 & 1.003 \\
		Exe Time Speedup & 1.07x & 1.05x & 1.30x & 3.38x & 4.92x & 1.08x & 20.45x \\
		
		\hline
	\end{tabular}
	}
 \vspace{-0.1in}
\end{table}





\iffalse
\begin{table}[!h]
	\centering  % 显示位置为中间
	\small
	\vspace{-0.1in}
	\caption{Benefit of PIM-aware Work Stealing in 3-CC.}  % 表格标题
	\label{tab:Benefit Of PIM-aware Work Stealing}  % 用于索引表格的标签
	%字母的个数对应列数，|代表分割线
	% l代表左对齐，c代表居中，r代表右对齐
	\vspace{-0.1in}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{c|c|c|c|c}  
	\hline
	    Graph & Stealing & Time (ns) & Avg Time (ns) &  Time Speedup\\
		\hline  % 表格的横线
	    \multirow{2}{*}{CI} & No & 5,572 & 4,565 & \multirow{2}{*}{1.19x} \\
	    & Yes & 4,701 & 4,597 & \\
	    \hline
		\multirow{2}{*}{PP} & No & 35,397 & 32,491 & \multirow{2}{*}{1.08x} \\
		& Yes & 32,675 & 32,572 & \\
		\hline
		\multirow{2}{*}{AS} & No & 244,929 & 217,084 & \multirow{2}{*}{1.12x} \\
		& Yes & 217,874 & 217,536 & \\
		\hline
		\multirow{2}{*}{MI} & No & 184,038 & 134,220 & \multirow{2}{*}{1.36x} \\
		& Yes & 135,411 & 135,089 & \\
		\hline
		\multirow{2}{*}{YT} & No & 407,856 & 253,625 & \multirow{2}{*}{1.44x} \\
		& Yes & 283,333 & 264,229 & \\
		\hline
		\multirow{2}{*}{PA} & No & 400,444 & 368,255 & \multirow{2}{*}{1.09x} \\
		& Yes & 371,445 & 370,555 & \\
		\hline
		\multirow{2}{*}{LJ} & No & 292,435 & 185,873 & \multirow{2}{*}{1.43x} \\
		& Yes & 203,874 & 190,579 & \\
		\hline
	\end{tabular}
	}
\end{table}
\fi

==> section/6_3_Comparison_Between_Real_Machine_and_Our_Simulator.tex <==
\subsection{Simulation Methodology Validation}
\label{subsec:compare real machine and simulator}

Due to the long execution time of the cycle-accurate simulator, for larger graphs, we sample the vertices $v_0$ in the first level during trace generation. The sample ratio is set so that each simulation can finish within ten hours. Other work using cycle-accurate simulation also adopt similar sampling methodology \cite{besta2021sisa}.
To ensure the accuracy of the sampling results, we record the pre-sampling and post-sampling execution times(Execution Time and Sample Time in Table \ref{tab:Graph Mining Systems Comparison 1 thread}) on the real machine and calculated the ratio of the two $r = Sample/Execution$. 
To avoid the overhead of OpenMP on real machines, we use a single thread to measure the performance in Table \ref{tab:Graph Mining Systems Comparison 1 thread}.
On our CPU simulator (similar configuration as the real machine), we measure the sample simulated time, and calculate $Estimated$ $Simulated$ $Time$ = $Sample$ $Simulated$ $Time$ / $r$.



%To show that the simulator is not biased, we compare the real machine results and the simulator results of the AutoMine algorithm under similar system parameters.
%To avoid the overhead of OpenMP on real machines, we use a single thread to measure the performance in Table \ref{tab:Graph Mining Systems Comparison 1 thread}.


% Due to the long execution time of the cycle-accurate simulator, for larger graphs, we sample the vertices $v_0$ in the first level.
% To ensure the accuracy of the sampling results, we ran the pre-sampling and post-sampling execution times (Execution Time and Sample Time in Table \ref{tab:Graph Mining Systems Comparison 1 thread}) on the real machine respectively, and calculated the ratio of the two $r = Sample/Execution$. 
% %We use $r$ to calculate the estimated simulated time for the whole execution. 
% Because we are using the same trace as the real machine after sampling, all execution times on our simulator are obtained by the formula $Estimated$ $Simulated$ $Time$ = $Sample$ $Simulated$ $Time$ / $r$.



We bold the real machine execution time (left) and our estimated simulator time (right) in Table \ref{tab:Graph Mining Systems Comparison 1 thread}.
Our simulator's reported time is on the same order of magnitude as the real machine, and the simulator reported time is slightly longer than the real machine. This demonstrate the sampling mechanism used in our evaluation is effective, efficient and unbiased.


%Therefore, our evaluation of PIMMiner using graph sample is fair.



% \iffalse
% \begin{table}[!h]
% 	\centering  % 显示位置为中间
% 	\small
% 	\vspace{-0.1in}
% 	\caption{Comparison Between Real Machine and Our Simulator And Sampling (one thread, /SEC.)}  % 表格标题
% 	\label{tab:Graph Mining Systems Comparison}  % 用于索引表格的标签
% 	%字母的个数对应列数，|代表分割线
% 	% l代表左对齐，c代表居中，r代表右对齐
% 	\vspace{-0.1in}
% 	\resizebox{\linewidth}{!}{
% 	\begin{tabular}{c|c|c|c|c|c|c|c}  
% 	\hline
% 	    Pattern & Graph & Total & Sample & Sample & Sample & Sample & Estimate\\
% 	    & & Time & Ratio & Time & /Total & Simulated Time & Simulated Time \\
% 		\hline  % 表格的横线
% 		\multirow{7}{*}{3-CC} & CI & \textbf{4.27E-04} & 1 & - & -  & 5.19E-04 & \textbf{5.19E-04}\\
% 		& PP & \textbf{3.77E-03} & 1 & - & - & 4.30E-03 & \textbf{4.30E-03} \\
% 		& AS & \textbf{4.39E-02} & 1 & - & - & 3.44E-02 & \textbf{3.44E-02}\\
% 		& MI & \textbf{2.96E-01} & 0.1 & 3.05E-02 & 0.103  & 3.69E-02 & \textbf{3.58E-01}\\
% 		& YT & \textbf{1.11} & 0.01 & 1.57E-02 & 0.012  & 3.03E-02 & \textbf{2.14}\\
% 		& PA & \textbf{3.56} & 0.01 & 4.31E-02 & 0.014  & 7.64E-02 & \textbf{6.31}\\
% 		& LJ & \textbf{20.33} & 0.001 & 2.24E-02 & 0.001 & 4.38E-02 & \textbf{39.75}\\
% 		\hline
% 		\multirow{7}{*}{4-CC} & CI & \textbf{4.36E-04} & 1 & - & - & 6.21E-04 & \textbf{6.21E-04}\\
% 		& PP & \textbf{3.79E-03} & 1 & - & - & 4.41E-03 & \textbf{4.41E-03} \\
% 		& AS & \textbf{2.38E-01} & 1 & - & - & 2.37E-01 & \textbf{2.37E-01}\\
% 		& MI & \textbf{5.26} & 0.1 & 4.57E-01 & 0.087 & 5.84E-01 & \textbf{6.73}\\
% 		& YT & \textbf{2.9} & 0.01 & 3.34E-02 & 0.012 & 8.14E-02 & \textbf{7.08}\\
% 		& PA & \textbf{4.17} & 0.01 & 5.02E-02 & 0.012 & 8.12E-02 & \textbf{6.74}\\
% 		& LJ & \textbf{120.41} & 0.001 & 1.00E-01 & 0.001 & 1.53E-01 & \textbf{183.95}\\
% 		\hline
% 		\multirow{7}{*}{5-CC} & CI & \textbf{4.70E-04} & 1 & - & - & 6.46E-04 & \textbf{6.46E-04}\\
% 		& PP & \textbf{3.79E-03} & 1 & - & - & 4.42E-03 & \textbf{4.42E-03} \\
% 		& AS & \textbf{1.21} & 1 & - & - & 1.68  & \textbf{1.68 }\\
% 		& MI & \textbf{181.24} & 0.001 & 1.80E-01 & 0.001  & 2.41E-01 & \textbf{242.43 }\\
% 		& YT & \textbf{4.51} & 0.001 & 7.49E-01 & 0.108  & 1.21 & \textbf{11.22}\\
% 		& PA & \textbf{6.97} & 0.01 & 2.31E-01 & 0.051  & 2.41E-01 & \textbf{4.69}\\
% 		& LJ & \textbf{3780} & 0.0002 & 5.61E-01 & 0.00015 & 1.22  & \textbf{8195.84}\\
% 		\hline
% 		\multirow{7}{*}{3-MC} & CI & \textbf{1.25E-03} & 1 & - & - & 1.31E-03 & \textbf{1.31E-03}\\
% 		& PP & \textbf{1.47E-02} & 1 & - & - & 1.32E-02 & \textbf{1.32E-02} \\
% 		& AS & \textbf{1.71E-01} & 1 & - & - & 1.41E-01 & \textbf{1.41E-01}\\
% 		& MI & \textbf{1.18} & 0.1 & 1.22E-01 & 0.103  & 1.27E-01 & \textbf{1.23 }\\
% 		& YT & \textbf{13.03} & 0.01 & 1.46E-01 & 0.011  & 2.38E-01 & \textbf{21.22 }\\
% 		& PA & \textbf{6.81} & 0.01 & 1.10E-01 & 0.016  & 2.17E-01 & \textbf{13.44 }\\
% 		& LJ & \textbf{84.47} & 0.001 & 8.22E-02 & 0.001  & 1.41E-01 & \textbf{145.05}\\
% 		\hline
% 	\end{tabular}
% 	}
% \end{table}
% \fi


\begin{table}[!h]
	\centering  % 显示位置为中间
	\small
%	\vspace{-0.1in}
	\caption{Comparison Between Real Machine and Our Simulator And Sampling (one thread, in seconds). }  % 表格标题
	\label{tab:Graph Mining Systems Comparison 1 thread}  % 用于索引表格的标签
	%字母的个数对应列数，|代表分割线
	% l代表左对齐，c代表居中，r代表右对齐
	\vspace{-0.1in}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{c|c|c||c|c|c|c|c}  
	\hline
	    Pattern & Graph & Execution & Sample & Sample & Sample & Sample & Estimated\\
	    & & Time & Ratio & Time & /Total ($r$) & Simulated Time & Simulated Time \\
		\hline  % 表格的横线
		\multirow{7}{*}{3-CC} & CI & \textbf{4.27E-04} & 1 & - & -  & 5.19E-04 & \textbf{5.19E-04}\\
		& PP & \textbf{3.77E-03} & 1 & - & - & 4.30E-03 & \textbf{4.30E-03} \\
		& AS & \textbf{4.39E-02} & 1 & - & - & 3.44E-02 & \textbf{3.44E-02}\\
		& MI & \textbf{2.96E-01} & 0.1 & 3.05E-02 & 0.103  & 3.69E-02 & \textbf{3.58E-01}\\
		& YT & \textbf{1.11} & 0.01 & 1.57E-02 & 0.012  & 3.02E-02 & \textbf{2.13}\\
		& PA & \textbf{3.56} & 0.01 & 4.31E-02 & 0.014  & 7.64E-02 & \textbf{6.31}\\
		& LJ & \textbf{20.33} & 0.001 & 2.24E-02 & 0.001 & 4.38E-02 & \textbf{39.75}\\
		\hline
		\multirow{7}{*}{4-CC} & CI & \textbf{4.36E-04} & 1 & - & - & 6.21E-04 & \textbf{6.21E-04}\\
		& PP & \textbf{3.79E-03} & 1 & - & - & 4.41E-03 & \textbf{4.41E-03} \\
		& AS & \textbf{2.38E-01} & 1 & - & - & 2.37E-01 & \textbf{2.37E-01}\\
		& MI & \textbf{5.26} & 0.1 & 4.57E-01 & 0.087 & 5.84E-01 & \textbf{6.73}\\
		& YT & \textbf{2.90} & 0.01 & 3.34E-02 & 0.012 & 8.14E-02 & \textbf{7.08}\\
		& PA & \textbf{4.17} & 0.01 & 5.02E-02 & 0.012 & 8.12E-02 & \textbf{6.74}\\
		& LJ & \textbf{120.41} & 0.001 & 1.00E-01 & 0.001 & 1.53E-01 & \textbf{183.95}\\
		\hline
		\multirow{7}{*}{5-CC} & CI & \textbf{4.70E-04} & 1 & - & - & 6.46E-04 & \textbf{6.46E-04}\\
		& PP & \textbf{3.79E-03} & 1 & - & - & 4.42E-03 & \textbf{4.42E-03} \\
		& AS & \textbf{1.21} & 1 & - & - & 1.68  & \textbf{1.68}\\
		& MI & \textbf{181.24} & 0.001 & 1.80E-01 & 0.001  & 2.85E-01 & \textbf{286.79}\\
		& YT & \textbf{6.97} & 0.001 & 7.49E-01 & 0.108   & 1.21 & \textbf{11.22}\\
		& PA & \textbf{4.51} & 0.01 & 2.31E-01 & 0.051  & 2.41E-01 & \textbf{4.70}\\
		& LJ & \textbf{3780} & 0.0002 & 5.61E-01 & 0.00015 & 1.22  & \textbf{8195.84}\\
		\hline
		\multirow{7}{*}{3-MC} & CI & \textbf{1.25E-03} & 1 & - & - & 1.31E-03 & \textbf{1.31E-03}\\
		& PP & \textbf{1.47E-02} & 1 & - & - & 1.32E-02 & \textbf{1.32E-02} \\
		& AS & \textbf{1.71E-01} & 1 & - & - & 1.41E-01 & \textbf{1.41E-01}\\
		& MI & \textbf{1.18} & 0.1 & 1.22E-01 & 0.103  & 1.27E-01 & \textbf{1.23 }\\
		& YT & \textbf{6.81} & 0.01 & 1.10E-01 & 0.016  & 2.17E-01 & \textbf{13.44}\\
		& PA & \textbf{13.03} & 0.01 & 1.46E-01 & 0.011 & 2.38E-01 & \textbf{21.22}\\
		& LJ & \textbf{84.47} & 0.001 & 8.22E-02 & 0.001  & 1.41E-01 & \textbf{145.05}\\
		\hline
	\end{tabular}
	}
\end{table}

